SOLO: Search Online, Learn Offline for Combinatorial Optimization Problems

We study combinatorial problems with real world applications such as machine scheduling, routing, and assignment. We propose a method that combines Reinforcement Learning (RL) and planning. This method can equally be applied to both the offline, as well as online, variants of the combinatorial problem, in which the problem components (e.g., jobs in scheduling problems) are not known in advance, but rather arrive during the decision-making process. Our solution is quite generic, scalable, and leverages distributional knowledge of the problem parameters. We frame the solution process as an MDP, and take a Deep Q-Learning approach wherein states are represented as graphs, thereby allowing our trained policies to deal with arbitrary changes in a principled manner. Though learned policies work well in expectation, small deviations can have substantial negative effects in combinatorial settings. We mitigate these drawbacks by employing our graph-convolutional policies as non-optimal heuristics in a compatible search algorithm, Monte Carlo Tree Search, to significantly improve overall performance. We demonstrate our method on two problems: Machine Scheduling and Capacitated Vehicle Routing. We show that our method outperforms custom-tailored mathematical solvers, state of the art learning-based algorithms, and common heuristics, both in computation time and performance.

==> abstract.tex <==
\begin{abstract}
We investigate a novel approach that combines reinforcement learning (RL) and planning to combinatorial optimization problems in offline and online settings.
As classical approaches are typically either compute-intensive or rely on approximations and are limited when dealing with stochastic systems or dynamically changing states, 
Conversely, learned policies should be well suited to deal with these effects while also allowing for compute compression via offline training.
Practically though, most existing RL solutions are still limited by either large or dynamically changing state-action spaces.
We frame the state-action space as a graph, allowing our trained policies to deal with arbitrary changes in a principled manner. 
Second, even when learned policies  work well in expectation, small deviations can have large negative effects in combinatorial settings. 
We mitigate these drawbacks by employing our graph-convolutional policies as non-optimal heuristics in a compatible search algorithm such as Monte Carlo Tree Search to significantly improve overall performance. 
We focus on two combinatorial problems: Machine Scheduling and  Capacitated Vehicle Routing and show that our method is competitive with custom-tailored mathematical solvers and outperforms both recently proposed learning-based algorithms and common heuristics.
\end{abstract}


==> acknowledgments.tex <==
\section*{Acknowledgments}
The authors would like to thank Erez Karpas and Alexander Shleyfman for their insights and improvements during the production of this manuscript.

==> algorithm_test.tex <==

{\SetAlgoNoLine

\begin{algorithm}
\caption{MCTS with pruned action search}\label{alg:mcts}
    \DontPrintSemicolon
    \SetKwFunction{Fupdate}{update\_tree}
    \SetKwFunction{Ftop}{top\_actions}
    \KwIn{State $S^{t}$, Environment $env$, $Q$-value estimator $\tilde Q$, random seed $seed$, rollout budget $n_{r}$, time budget $t_{max}$, prune limit $k$, state visits counter $n_s(\cdot)$, state-action visits counter $n_{s,a}(\cdot,\cdot)$, Search Tree estimator $Q^{\mathcal{T}}$}
    env.set\_seed(seed) \\
    
    \For{$r \leftarrow 1,\ldots,n_{r}$}
    {
        \If{elapsed\_time() $> t_{max}$}{
            break
        }  
        $s \leftarrow$ env.set\_state$(S^t)$ \\
        $done, \rho \leftarrow false, [] $\\
        $t_{out}\leftarrow\infty$\\
        $t\leftarrow 0$\\
        \While{not done}
        {
            $t\leftarrow t+1$\\
            $top\_Q \leftarrow$ get\_top\_actions$(s, \tilde{Q}, k)$ \\
            \If{$n_s\left(s\right) == 0$}{
                \tcp*{action with max. Q-value}
                $a \leftarrow \arg_a\max [top\_Q] $\\
                $t_{out}\leftarrow \min(t, t_{out})$
            }
            \Else{
                $q_{UCB} \leftarrow \{\}$ \\
                \For{$a, q_a \in top\_Q$}{
                    $q_{UCB}\left[a\right] \leftarrow Q^{\mathcal{T}}(s, a) + \beta \sqrt{\frac{\log{n_s(s)}}{n_{s,a}(s,a)}}$
                }
                $a \leftarrow \arg_a\max [q_{UCB}]$ \\
            }
            $r, s', done  \leftarrow$ env.step$(a)$ \\
            $\rho\left[t\right]\leftarrow\left< s, a, r \right>$ \\
            $s \leftarrow s'$ \\
            update\_tree$(\rho, n(\cdot), n(\cdot,\cdot), t_{out})$
        }
    }
    a\_chosen = $\arg_a\max Q^{\mathcal{T}}\left(S^t, a\right)$ \\
  \Return a\_chosen \\
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\Ftop{s, \tilde{Q}, k}}{ \\
%             $Q \leftarrow \tilde{Q}(s)$  \\
%             \KwRet{top-$k$ tuples in $Q$ by their value estimates.}}
  \SetKwProg{Fn}{Def}{:}{}
  \Fn{\Fupdate{$\rho, n_s, n_{s,a}, Q^{\mathcal{T}}, t_{out}$}}{ \\
    $\overline{r} \leftarrow 0$ \\
    \For{$i \leftarrow \left|\rho\right| \text{ to } 1$}{
        $s, a, r \leftarrow \rho[i]$ \\
        $\overline{r} \leftarrow r + \gamma \overline{r}$ \\
        \If{$i>t_{out}$}{continue}
        $n\left(s\right)\leftarrow n\left(s\right)+1$ \\
        $n\left(s,a\right)\leftarrow n\left(s,a\right)+1$ \\
        $Q^{\mathcal{T}}\left(s, a\right) \leftarrow \frac{n\left(s,a\right)-1}{n\left(s,a\right)}Q^{\mathcal{T}}\left(s, a\right) + \frac{1}{n\left(s,a\right)} \overline{r}$
    }}
\end{algorithm}
}

==> benchmark_explanation.tex <==
\subsection{Benchmark Problems}\label{sec:Benchmark Problems}
The following section introduces offline and online versions of the problem which we tested our approach on.

\subsubsection{The Capacitated Vehicle Routing Problem}
We consider a simplified version of the Capacitated Vehicle Routing problem (CVRP) introduced by Dantzig and Ramser~\cite{dantzig59}. There is a  set $N = \{ 1,\ldots,n \}$ of customers with individual demands $\{d_i \}_{i=1,\ldots,n}$ for a single commodity, and locations $\{p_i \}_{i=1,\ldots,n}$. The commodity is located at a depot $o$, and is to be transported from it to the customers so as to meet their demand by a vehicle of capacity $C^*$ (for feasibility, we assume that $d_i \leq C^*$ for all $i \in N$). There is a function $c(p, p')$ that prescribes the cost of travelling from location $p$ to location $p'$. A \textit{tour} consists of a path,  $\tau = (p_1 = o, \ldots, p_{n_{\tau}} = o)$, in which the vehicle's load does not exceed its capacity and satisfies the demands of the customers along it. The \textit{cost} of the tour $\tau$ is simply the total cost of travelling from along it: $c(\tau) = \sum_{i=1,\ldots,n_{\tau}-1}c(p_i, p_{i+1})$.

\paragraph{Online CVRP} 
We consider an online version, in which the customers arrive at times sampled from a distribution, while the vehicle is touring along the customers and depot. A decision point occurs when the vehicle arrives at its next target location,  and there is at least one available customer.\footnote{Note that that travel time between customers varies according to the distances between them, and thus one or more customers may arrive during the vehicle's travel.} 

\subsubsection{Parallel Machine Scheduling} (PMSP)
We consider (offline) scheduling problems \cite{KRAMER2019} where a number of jobs $N = \{ 1,\ldots,n \}$ are to be processed by a set of identical machines $M = \{ 1,\ldots,m \}$. Jobs are characterized by their classes $\{s_i \}_{i=1,\ldots,n}, s_i \in \{1, \dots, s \}$, processing time $\{p_i \}_{i=1,\ldots,n}$, and weights $\{w_i \}_{i=1,\ldots,n}$. Each machine can only process one job at a time and will take $p_i$ time units to complete it. Whenever two jobs $i, j$ are processed consecutively on a single machine, the setup of the machine might need to be changed, which incurs a time penalty (i.e., setup time) of $f(s_i, s_j)$, where $f(s_i, s_i) = 0$.



\paragraph{Online PMSP}
Additional jobs can arrive at a finite number of points in time (arrival intervals) in the online settings. The number of arriving jobs at the start of each interval is determined by an arrival distribution for each class (e.g., Poisson).


==> comparison_table.tex <==
\begin{table}[t!]
% \label{sample-table}
\caption{Related Work Classification - The Problem Solved are Satisfiability (SAT), Maximal Independent Set (MIS), Minimum Vertex Cover (MVC), and Maximal Clique (MC), Minimum Vertex Cover (MVC), Maximum Cut (MC), Traveling Salesperson (TSP), Job Shop Problem (JSP), Generalized Independent Set Problem (GISP), Set Cover (SC), Combinatorial Auction (CA), Maximum Independent Set (MIS), Vehicle Routing Problem (VRP)}
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccr}
\toprule
\textsc{Work} & \textsc{Problems Solved} & \textsc{Method} \\
\midrule
%Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
%Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Zhuwen et al. 2018 \cite{Zhuwen2018}         & SAT, MIS, MVC, MC    & SL \\
Khalil et al. 2017 \cite{KhalilEtAlNIPS2017} & MVC, MC, TSP         & RL \\
Kool et al. 2019 \cite{Kool2019ICLR}       & TSP                  & RL \\
Mao et al. 2019 \cite{MaoEtAl2019}        & JSP                  & RL \\
Waschneck et al. 2018 \cite{Waschneck2018a}\hspace{-1em}     & JSP                  & RL \\
Khalil et al. 2017 \cite{KhalilEtAlNIPS2017} & GISP                 & SL \\
Gasse et al. 2019 \cite{GasseEtal2019}      & SC, CA, MIS          & SL \\
Chen et al. 2019 \cite{chen2019learning}   & VRP, JSP, SAT        & RL \\
\bottomrule
\end{tabular}
% \end{sc}
\label{sample-table}
\end{small}
\end{center}
\end{table}

==> dqn_table.tex <==
\begin{table}[ht]
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{l*4l}
        %\toprule
        \multirow{2}{*}{\textbf{Parameter}} & \multicolumn{2}{c}{\textbf{PMS}} & \multicolumn{2}{c}{\textbf{CVRP}} \\ 
        & Offline & Online & Offline & Online \\
        %\midrule
        total time steps                     & $1e^6$ & $1e^6$ & $1e^6$ & $1e^6$ \\
        target network update frequency     & $5e^3$ & $5e^3$ & $5e^3$ & $5e^3$ \\
        initial random steps                & $5e^3$ & $5e^3$ & $5e^3$ & $5e^3$ \\
        learning starts $t$                 & $5e^3$ & $5e^3$ & $5e^3$ & $5e^3$ \\
        train frequency                     & $1$ & $1$ & $1$ & $1$ \\
        discount $\gamma$                   & $1.0$ & $0.9$ & $1.0$ & $1.0$ \\
        batch size                          & $32$ & $32$ & $128$ & $128$ \\
        replay buffer size                  & $5e^3$ & $5e^3$ & $5e^3$ & $5e^3$ \\
        prioritized replay $\alpha$         & $0.0$ & $0.0$ & $25e^{-3}$ & $25e^{-3}$ \\
        prioritized replay $\beta_0$        & $0.4$ & $0.4$ & $0.4$ & $0.4$ \\
        prioritized replay $e$              & $1e^{-6}$ & $1e^{-6}$ & $1e^{-6}$ & $1e^{-6}$ \\
        exploration fraction                & $0.3$ & $0.3$ & $0.1$ & $0.1$ \\
        exploration final                   & $0.1$ & $1e^{-4}$ & $1e^{-4}$ & $1e^{-4}$ \\
        learning rate                       & $1e^{-3}$ & $1e^{-3}$ & $1e^{-3}$ & $1e^{-3}$ \\
        learning rate $e$                   & $0.0$ & $0.0$ & $0.1$ & $0.1$ \\
        gradient norm clipping              & $2e^2$ & $2e^2$ & $2e^2$ & $2e^2$ \\
        double $Q$                          & \texttt{false} & \texttt{false} & \texttt{false} & \texttt{false} \\
        dueling                             & \texttt{false} & \texttt{false} & \texttt{true} & \texttt{true} \\
        $n$ step reward estimation          & $1$ & $1$ & $1$ & $1$ \\
        %\bottomrule
    \end{tabular}%
    }
    \caption{Training DQN hyper parameters used for all problems}\label{tab:DQNParams}
\end{table}

==> evaluation.tex <==
\section{Evaluation}\label{sec:evalutaion}
We test SOLO on the problems described in \autoref{sec:problem}. With few changes and little hyper-parameter tuning we achieve competitive results in the online problem without degrading the offline results.

\subsection{Capacitated Vehicle Routing Problem}
We apply our method to two variants of the Vehicle Routing problem. In the offline case, we consider the same setting as previous work \cite{chen2019learning, Kool2019ICLR, NIPS2018_nazari} and consider three scenarios with $N \in \{20,50,100\}$ customers and vehicle capacity $C \in \{30,40,50\}$, respectively.
The customers and the depot positions are uniformly sampled from the unit square, while the demands are sampled from a discrete uniform distribution $U[1, 10]$. 
Each setting is represented as a graph where the vehicle, depot and customers are nodes and edges are possible routes (see \autoref{app:training} for more details on the features used).
%This graph is then used for training our model similar to the scheduling problem.
 
For evaluation, we compare our results to the following baselines: a trained neural rewriter model \cite{chen2019learning}, the two strongest baselines reported by Nazari et al.~\cite{NIPS2018_nazari} (Savings and Sweep), Google’s OR-Tools, and the naive Distance Proportional baseline. In the latter baseline, each valid customer (whose demand is lower than the current capacity) is selected with probability proportional to its distance from the vehicle. More details about the baselines can be found in \autoref{app:baselines}, in particular about the fact that the training time for all neural models was limited to 24 hours.
%\chr{if needed part of this paragraph about the baselines can go into the appendix and here we can just write the names of the methods}
We evaluate the trained Q-net alone and with MCTS (SOLO), allowing MCTS $10$ seconds to optimize each decision. In addition, to better understand the contribution of our model to MCTS, we replace it with our naive baseline, Distance Proportional (MCTS+distance) and compare all the results.


\paragraph{Online Capacitated Vehicle Routing:} In this case we assume the same sizes and capacities as before and introduce a starting time for each customer. The positions and times of customers are now sampled from a Truncated Gaussian Mixture Model (TGMM) (see Appendix \ref{app:evaluations} for a full description of the distributions). We choose to change the position distribution in order to better show SOLO's strength in learning sample distribution (In the offline setting where baselines exist we choose to use the same distribution as in the baselines for easy comparison).
%\chr{add more specific explanation about distribution in the appendix}
%
As described by Jaillet et al.\ \cite{online_vrp_survey} the known algorithms for online routing problems are used to minimize the competitive ratio which is a more theoretical worst-case measure and less  suitable in more practical scenarios. For this reason, we choose to compare our results with the offline algorithms while running them in a quasi-offline manner (every time the vehicle returns to the depot, we re-run the algorithms while including only currently opened customers in the observation; see \autoref{app:baselines}).
Unlike the offline problem, we run MCTS with a truncated horizon where in each rollout a limited number of future customers is sampled. Given the limited computing time, this method allows for a good balance between planning for the future on the one hand, but also seeing a broad view of the current state and possible actions.

 \begin{figure}[t]
    \centering
    \subfloat[offline routing 50]{%
        \includegraphics[trim=0 25 0 0,width=0.5\columnwidth]{plots/static_vrp50_10sec.png}\label{fig:offline_vrp50}
    }
    \subfloat[online routing 50]{%
        \includegraphics[trim=0 25 0 0, width=0.5\columnwidth]{plots/dynamic_vrp50_10sec_new.png}\label{fig:online_vrp50}
    }
    \caption{Results for the offline and online CVRP benchmark setting on $50$ instances. Lower values indicate better performance. For each approach $a$ and instance $i$, the plot shows the relative disadvantage to OR-Tools calculated as $\mathrm{mean}_i((v_a(i) - v_\mathrm{OR-Tools}(i)) / v_\mathrm{OR-Tools}(i))$.}
    \label{fig:results_vrp}
\end{figure}

%\jo{Switch at least some of the occurrences of ``our method'' and ``our algorithm'' to SOLO.} %\chr{done...}
In \autoref{fig:results_vrp} we see results for the VRP 50 setting in both the offline and online problem (\autoref{app:evaluations} contains results for other settings). In the offline problem (Figure~\ref{fig:offline_vrp50}) Q-net is close to OR-Tools and achieves better results when combined with MCTS and the full capacity of SOLO is used. In addition, compared to neural rewriter, our results are better for all episodes. The savings algorithm achieves slightly better results than SOLO (showing, an average $4\%$ gap compared to  $2\%$ in our case). As savings is a problem specific heuristic, it is therefore expected to achieve good results on the offline problem. However, as we can see in Figure~\ref{fig:online_vrp50} fails to excel in the online setting.
%\fr{@Chana I think the previous sentence is a little confusing. Can you rephrase it?}\chr{what about this?}\fr{good in general, but I think there are some missing words now}.
In the online problem (Figure~\ref{fig:online_vrp50}) Q-net alone out preforms the learning algorithm and problem specific heuristics. Also, our complete algorithm, SOLO, achieves overall better results (Q-net alone achieves an average gap of $5\%$ while SOLO is $23\%$ better than OR-Tools). In addition MCTS alone improves the distance heuristic drastically, showing better results for all seeds run and proving that algorithms with the ability to predict online the distribution of future customers are more successful than ones trying to solve only the current offline problem.
Note that in all VRP cases SOLO+prune did not show any improvement on SOLO alone and we decided not to include this in the plots.

\subsection{Parallel Machine Scheduling}
%We evaluate the described method on several parallel machine scheduling problems.

First, we consider the offline version of the scheduling problem where the set of jobs is completely known, and for which our baselines were designed. We consider a case with $80$ jobs, $3$ machines, and $5$ job classes.
We represent a state as a bipartite graph of job and machine nodes, where the job and machine features are represented as node features, and edges are labeled with setup times. See \autoref{app:training}.
%\ml{maybe we should skip this sentence completely and refer reader to the appendix immediately?} \fr{I would argue against that. We need to give at least a minimal explanation otherwise the paper would no be self-contained.}
We train a model on problems where we sample job processing times from discrete $U[1, 100]$, setup times between different classes from $U[1, 50]$, and job weights from $U[1, 10]$.
%\ml{square brackets are confusing with citations} \fr{square brackets are also common notation for intervals. I think it's unambiguous since you normally have whitespace before a citation.}
%
We then evaluate it on a public set of benchmark problems that uses same ranges for job features \cite{Liao2012}.
% \jo{The following sentence introduces more questions. If it wasn't trained on the problems in the benchmark, then what was it trained on?} \fr{I reordered the section to present the offline setting first. For that, I also put the sentence that explains the job feature ranges here. That should answer the questions.}
We compare against the weighted shortest processing times first heuristic (WSPT), neural rewriter \cite{chen2019learning}, and the CPOptimizer of IBM ILOG CPLEX Optimization Studio V12.9.0.
%\footnote{\url{https://www.ibm.com/support/knowledgecenter/en/SSSA5P\_12.9.0/ilog.odms.studio.help/Optimization_Studio/topics/COS_home.html}} (CPLEX).
More details can be found in \autoref{app:baselines}.
We also analyze the contributions of our Q-net model and the MCTS component to the overall performance of SOLO by showing Q-net performance with and without MCTS, and by replacing the Q-net model with WSPT in MCTS (MCTS+WSPT). In all cases, we give MCTS $10$ seconds to optimize each decision.
Figure \ref{fig:scheduling-static} shows that although our approach does not specifically target offline problems, it is on par with the optimized baseline CPLEX in this challenging case, indicating that similarly specialized code would potentially to outperform even CPLEX. 
%, showing that it does not sacrifice quality on static problems \jo{static or dynamic?} in favor of performance in dynamic cases. \fr{removed this half-sentence because it no longer makes sense to put here.}

\begin{figure}[t]
    \centering
    \subfloat[offline scheduling 80]{%
        \includegraphics[trim=0 20 0 0,width=0.5\columnwidth]{plots/liao-n80.png}
        \label{fig:scheduling-static}
    }
    \subfloat[online scheduling 80]{%
        \includegraphics[trim=0 20 0 0,width=0.5\columnwidth]{plots/dynamic-m3.png}
        \label{fig:scheduling-dynamic}
    }
    \caption{Results for the offline and online scheduling benchmark setting on 50 instances each. Lower values indicate better performance. For each approach $a$ and instance $i$, the plot shows the relative disadvantage to CPLEX calculated as $\mathrm{mean}_i((v_a(i) - v_\mathrm{CPLEX}(i)) / v_\mathrm{CPLEX}(i))$.}
    \label{fig:scheduling}
\end{figure}


\paragraph{Online Scheduling:} Next, we define an online setting with $80$ jobs in expectation and $5$ job classes. There are $3$ machines, and the jobs arrive in $16$ intervals of length $130$ time units, each. Jobs arrive according to Poisson distributions, where the frequency of the $i$-th class is proportional to $1/i$. The problem parameters were chosen so as to not overload the machines in steady state on the one hand,
%(to preserve a reasonable backlog of jobs),
while maintaining relatively low levels of idleness.
%\jo{This sentence is too colloquial. Maybe ``to preserve a reasonable backlog of jobs'', or something like that.} \fr{done}
%\jo{Remove this sentence to save spacel; the intentions here should be clear.} This ensures that the considered setting does not produce trivial problems.
We again train a Q-net model and evaluate its performance with $50$ random seeds.
We also again run MCTS with a truncated horizon that limits the number of arriving jobs.
As the neural rewriter and CPLEX baselines are intended for offline settings, we let them recompute schedules for every decision. The results are depicted in Figure \ref{fig:scheduling-dynamic}. It is apparent that Q-net outperforms WSPT on average, and is thus a good choice when the time per step is limited. When compute time becomes available, MCTS significantly improves the solution
%\chr{if we want to leave this sentence here i think we need to write a bit more, clearly adding time to MCTS will bring better results} \fr{We're contrasting MCTS@10s with pure G graphnet alone}
In particular, it consistently outperforms WSPT in all problem instances (see \autoref{app:evaluations}). Our approach performs mostly on par with CPLEX, with slight advantages for either on different instances. Neural rewriter generally improves upon WSPT, but does not reach Q-net performance.
More results on additional settings are shown in \autoref{app:evaluations}.
%\ml{previously started from lowercase} 


%As indicated by \autoref{fig:static-n20} and \autoref{fig:static-n80}, our approach also compares favorably in this case. Notably, the Q graphnet policy scales well to the 80 job case and still outperforms WSPT, especially in combination with MCTS, which further increases the advantage \fr{verify this claim}. Neural rewriter on the other hand cannot improve schedules beyond WSPT performance, and CPLEX often fails to find any solution at all within the 10s time limit \fr{verify}.

% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \label{fig:static-n20}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \label{fig:static-n80}
% \end{figure}

%We also evaluate the model trained on the 20 job static setting on a public set of benchmarks where the optimal solution quality is known \cite{KRAMER2019}. \ml{highlight here that the model wasn't trained on benchmark environment} 

%\fr{story: show dynamic cases; static cases serve as an example for one interval in the dynamic cases. If we take away the uniqueness of our dynamic setting and compare on classical settings, we are still doing well (n=20 static, n=20 static Liao). As the problems become larger n=80, our approach becomes better than CPLEX in the given time frame, while staying better than WSPT, especially in combination with MCTS. Compared to static solvers, we have the ability to learn stochastic patterns.}


%\fr{everyone}
%\begin{itemize}
    %\item Two static settings where the expected number of jobs is 20 and 80, respectively, the number of machines is $3$, and the number of job classes is $5$. 
%    \item Two dynamic settings where expected total number of jobs is 80 and the number of job classes is $5$. In the first setting, there are 3 machines, and the jobs arrive 16 intervals that are each 130 time units long. In the second setting, there are 10 machines, and the jobs arrive in 60 intervals of 10 time units each. \fr{add how the interval duration was chosen} The duration of each interval is chosen so that ?????.
%\end{itemize}
%In all cases, we sample job processing times uniformly between 1 and 100, setup times between different classes from 1 to 50, and job weights from 1 to 10, following the ranges used by \citet{KRAMER2019}.
%For each configuration we train a model and evaluate its performance on the same configuration with 50 random seeds. 
%We also evaluate the model trained on the 20 job static setting on a public set of benchmarks where the optimal solution quality is known \cite{KRAMER2019}. 
%The baseline approaches can be applied directly in the static settings. 

%\fr{Add 2 violin plots for static settings}

%\fr{Add violin plot for evaluation on Liao benchmark with n=20, including optimal values.}

%\fr{Add 2 violin plots for dynamic settings}





==> evaluation_extended.tex <==
\section{Evaluation}\label{sec:evalutaion_extended}
% In this section we demonstrate our method --- SOLO on the two problems described in \autoref{sec:problem}. 
% For every problem type, We used an identical sets of hyperparameters and the same Q-net architecture, for all its variants.
% We demonstrate satisfying results for online settings of both problems without sacrificing on offline performance. 
%We test SOLO on the problems described in \autoref{sec:problem}. With little changes and small hyper-parameter tuning between the different problems we managed to achieve satisfying results in both online settings without degrading the offline results.
%We evaluate SOLO on the problems described in \autoref{sec:problem}. 
% With few changes and little hyperparameter tuning we achieve competitive results in online problems without degrading the offline results.
%For both problems we use the same set of hyperparameters and the same Q-net architecture for all its variants.
%We demonstrate competitive results for online settings of both problems without sacrificing on %offline performance.
We evaluate SOLO on the problems described in \autoref{sec:problem}. With little changes and small hyper-parameter tuning between the different problems (CVRP and scheduling) we managed to achieve competitive results in both online settings without degrading the offline results. 
%\ml{That's really ambiguous phrasing. Little changes and HP tuning for what: for two different problems, or for online/ofline case, or for different problem sizes?} \fr{The reader will find out by continuing to read, so no need to be more specific here.}
%\ml{correct me if I'm wrong but we're never mentioning hyperparams again till the appendix}
%\fr{that might be, but we refer to these appendices}
%\ml{I would rephrase it, it takes one sentence and maybe up to 10 mins, but I think that making it cleat that our method is able to achieve performance for all problem variations with the same set of prarams is important}
%\fr{all right, make a proposal. As I said, let's try to finish this.}

% Plan:
% \begin{itemize}
%     \item Focus on dynamic settings
%     \item include additional experiment with longer search
%     \item argue about extend-ability to bigger problem sizes
%     \item give static results only in form of a table 
% \end{itemize}

\subsection{Capacitated Vehicle Routing Problem}
% We apply our method to two variants of the Vehicle Routing problem. 
% For the offline case, we consider the same setting as previous work \cite{chen2019learning, Kool2019ICLR, NIPS2018_nazari} and consider three scenarios with $N \in \{20,50,100\}$ customers and vehicle capacity $C \in \{30,40,50\}$, respectively.
% The customers and the depot positions are uniformly sampled from the unit square, while the demands are sampled from a discrete uniform distribution $U[1, 10]$. 
% Each setting is represented as a graph where the vehicle, depot and customers are nodes and edges are possible routes (see \autoref{app:training} for more details on the features used).
%This graph is then used for training our model similar to the scheduling problem.
%\jo{The location and capacity distributions are now omitted.}
%\ml{They moved to the static paragraph}
%\fr{Where? I don't see anything about distributions in the offline part}
%\ml{sorry, accedently commented them}
For both online and offline cases, we consider the same setting as previous work \cite{chen2019learning, Kool2019ICLR, NIPS2018_nazari} and consider three scenarios with $N \in \{20,50,100\}$ customers and vehicle capacity $C \in \{30,40,50\}$, respectively.
We compare our results to the following baselines: a trained neural rewriter model \cite{chen2019learning}, the two strongest baselines reported by Nazari et al.~\cite{NIPS2018_nazari} (Savings and Sweep), Google’s OR-Tools, and the naive Distance Proportional baseline. 
In the latter baseline, each valid customer (whose demand is lower than the current capacity) is selected with probability proportional to its distance from the vehicle. 
See \autoref{app:baselines} for details. %, in particular about the fact that the training time for all neural models was limited to 24 hours.
We evaluate the trained Q-net alone and with MCTS (SOLO). 
In addition, to better understand the contribution of our model to MCTS, we replace it with our naive baseline, distance proportional (MCTS+distance) and compare all the results.
We used the same training time for the Q-net and neural rewriter for all problem sizes.
MCTS and OR-Tools were given $10$ seconds to optimize each decision.
For additional details please see \autoref{app:training}.

\paragraph{Online Capacitated Vehicle Routing}
% \ml{adjustements specific to online setting}
In this case we introduce an arrival time for each customer. 
% \ml{problem setting?} \fr{matter of taste}
%\fr{I changed "starting" to "arrival" to be consistent with the rest of the paper and the related work}
The positions and times of customers are sampled from a Truncated Gaussian Mixture Model (TGMM) (see Appendix \ref{app:evaluations} for a full description of the distributions). 
We use this position distribution in order to better show SOLO's strength in learning sample distribution. 
%\ml{I would leave my previous formulation for this sentens (which I cannot find anymore :( ) which was formulating this in: "implicitly incorporating the distribution into learning process". I guess that "learning sample distribution" is quite a bold statement given that we can't prove that.}
%\fr{Sorry Maksym, but we can't keep editing back and forth. Obviously someone had a different opinion and we need to compromise.}
%(in the offline setting where baselines exist we use the same distribution as in previous work for easy comparison).
As described by Jaillet et al.\ \cite{online_vrp_survey} the known algorithms for online routing problems are used to minimize the competitive ratio, which is a more theoretical worst-case measure and less suitable in more practical scenarios. 
For this reason, we choose to compare our results with the offline algorithms discussed in the previous section, while running them in a quasi-offline manner (every time the vehicle returns to the depot, we re-run the algorithms while including only currently opened customers in the observation; see \autoref{app:baselines}).
%\ml{also here I would replace parentheses with "i.e." as it was previously.}
%\fr{again, this is a matter of taste and I don't want to edit back and forth.}
In this variant of the problem, we run MCTS with a truncated horizon where in each rollout a limited number of future customers is sampled. 
Given the limited computing time, this method allows for a good balance between planning for the future on the one hand, but also seeing a broad view of the current state and possible actions.

% Location distribution is changed (comparing to classical problem formulation) in order to better demonstrate SOLO's ability to implicitly incorporate the sample distribution into learning.
%\fr{The reader does not know what the classic problem formulation is at this point, so we need to rephrase the previous sentence} \ml{yes}
% (In the offline setting where baselines exist we choose to use the same distribution as in the baselines for easy comparison). 
% The known algorithms for online routing problems are used to minimize the competitive ratio, which is a more theoretical worst-case measure and less suitable in more practical scenarios \cite{online_vrp_survey}. 
% Therefore, we compare our results with the offline algorithms while running them in a quasi-online manner: every time the vehicle returns to the depot, we re-run the algorithms while including only currently opened customers in the observation (see \autoref{app:baselines}).
% We run MCTS with a truncated horizon where in each rollout a limited number of future customers is sampled. 
% Given the limited compute time, this method allows for a good balance between planning for the future on the one hand, but also seeing a broad view of the current state and possible actions.

% \begin{wrapfigure}{r}{.5\textwidth}
%     \begin{minipage}{\linewidth}
%         \centering\captionsetup[subfigure]{justification=centering}
%         \includegraphics[width=\linewidth]{plots/dynamic_vrp20_10sec_new.png}
%         \subcaption{online routing 20}
%         \label{fig:5a}\par\vfill
%         \includegraphics[width=\linewidth]{plots/dynamic_vrp50_10sec_new.png}
%         \subcaption{online routing 50}
%         \label{fig:5b}
%         \includegraphics[width=\linewidth]{plots/dynamic_vrp100_10sec_new.png}
%         \subcaption{online routing 100}
%         \label{fig:5c}
%         \includegraphics[width=\linewidth]{plots/dynamic_vrp100_20sec_new.png}
%         \subcaption{online routing 100 (timeout 20)}
%         \label{fig:5c}
%     \end{minipage}
% \caption{Figure}\label{fig:5}
% \end{wrapfigure}
\begin{figure}[t]
% \begin{wrapfigure}{R}{.4\textwidth}
    \centering
    \subfloat[online routing 20]{%
        \includegraphics[trim=0 20 0 0, width=.5\columnwidth]{plots/dynamic_vrp20_10sec_new.png}\label{fig:online_vrp20_extended}
    } 
    \subfloat[online routing 50]{%
        \includegraphics[trim=0 20 0 0, width=.5\columnwidth]{plots/dynamic_vrp50_10sec_new.png}\label{fig:online_vrp50_extended}
    }\\[-2ex]
    \subfloat[online routing 100]{%
        \includegraphics[trim=0 20 0 0, width=.5\columnwidth]{plots/dynamic_vrp100_10sec_new.png}\label{fig:online_vrp100_extended}
    } 
    \subfloat[online routing 100 (timeout 20s)]{%
        \includegraphics[trim=0 20 0 0, width=.5\columnwidth]{plots/dynamic_vrp100_20sec_new.png}\label{fig:online_vrp100_to20_extended}
    }
    \smallcaption{
    Results for the online CVRP benchmark of different sizes on $50$ random instances. 
    Lower values indicate better performance. 
    For each approach $a$ and instance $i$, the plot shows the relative disadvantage to OR-Tools calculated as $\mathrm{mean}_i((v_a(i) - v_\mathrm{OR-Tools}(i)) / v_\mathrm{OR-Tools}(i))$.}
    \label{fig:results_vrp}
    \vspace{-1.5em}
% \end{wrapfigure}
\end{figure}
% \ml{result discussion goes here}
% \autoref{fig:results_vrp} demonstrates the results of evalutaion.
As shown in \autoref{fig:results_vrp} (a, b, c), for every problem size of the online CVRP problem, SOLO achieves the best performance.
% Q-net alone outperforms the Neural Rewriter, which additionally uses search for solution refinement, for smaller problems and is marginally worse for the biggest problem.
% That, considering that the bigger problems are notably more challenging (the search tree grows exponentially and the state-action space grows quadratically), demonstrates the scalability of the offline SOLO part.
% \ml{three above lines can be either changed or removed}
%That explains the relative performance decrease comparing to the OR-Tools baseline with the increasing problem size.
%\fr{We need to avoid that this sounds as if OR-Tools scales better with problem size.} 
%\ml{yes, agreed, but I've tried to address that in next two sentences}
% It can be observed that performance of Q-net alone following the same pattern, which might indicate that the Q.
%We performed additional experiment with extended search timeout for MCTS.
%As demonstrated \autoref{fig:results_vrp} (d) SOLO can better utilize the additional search time to comparing to OR-Tools.
%\fr{in fact OR-Tools does not seem to benefit at all from additional time. Its performance relative to the non-search methods Q-net, savings, etc. does not change. OR-Tools seems to either (1) be stuck in a local optimum, or (2) has reached the best that an offline algorithm can do.}
%\ml{rewriting is needed}
OR-Tools shows good scaling behaviour with increasing problem size, although it still barely matches SOLO for the largest problem size. We further investigate the scaling behaviour by increasing the search time. As is apparent from \autoref{fig:results_vrp} (d), SOLO utilizes the additional search time well, while OR-Tools does not seem to benefit at all. Its performance relative to the non-search methods like Q-net does not change. It is unclear whether OR-Tools found a local optimum or the global optimum achievable by offline approaches.
%\jo{Switch at least some of the occurrences of ``our method'' and ``our algorithm'' to SOLO.} %\chr{done...}
% In \autoref{fig:results_vrp} we see results for the VRP 50 setting in both the offline and online problem (results for other settings of the problem can be found in \autoref{app:evaluations}). 
% In the offline problem (Figure~\ref{fig:offline_vrp50}) Q-net is close to OR-Tools and achieves better results when combined with MCTS and the full capacity of SOLO is used. 
% In addition, compared to neural rewriter, the other learning method, our results are better for all episodes. 
% The savings algorithm achieves slightly better results than SOLO (showing, an average $4\%$ gap compared to  $2\%$ in our case). As savings is a problem specific heuristic, it is therefore expected to achieve good results on the offline problem. However, as we can see in Figure~\ref{fig:online_vrp50} fails to excel in the online setting.
%\fr{@Chana I think the previous sentence is a little confusing. Can you rephrase it?}\chr{what about this?}\fr{good in general, but I think there are some missing words now}.
% In the online problem (Figure~\ref{fig:online_vrp50}) Q-net alone out preforms the learning algorithm and problem specific heuristics. 
% Also, our complete algorithm, SOLO, achieves overall better results (Q-net alone achieves an average gap of $5\%$ while SOLO is $23\%$ better than OR-Tools). 
% In addition MCTS alone improves the distance heuristic drastically, showing better results for all seeds run and proving that algorithms with the ability to predict online the distribution of future customers are more successful than ones trying to solve only the current offline problem.
% Note that in all VRP cases SOLO+prune did not show any improvement on SOLO alone and we decided not to include this in the plots.
\paragraph{Offline Capacitated Vehicle Routing}\label{par:offline}
\begin{wraptable}{R}{.6\textwidth}
    \vspace{-1.3em}
    \smallcaption{Relative advantage to OR-Tools baseline for offline CVRP problems on $50$ random instances. Lower values indicate better performance.}
    \label{tab:cvrp_static}
    \tiny
    \centering
    \begin{tabular}{l*3c}
        \toprule
        baseline & VRP 20 & VRP 50 & VRP 100  \\ 
        \midrule
        Uniformly Random        & -13.21 (107.51\%) & -30.58 (167.52\%)         & -58.84 (230.13\%) \\
        Distance Proportional   & -10.43 (63.65\%)  & -24.36 (113.39\%)         & -47.59 (167.38\%) \\
        Savings                 & -6.35 (-1.04\%)   & \textbf{-11.03 (-3.98\%)} & \textbf{-16.51 (-7.94\%)} \\
        Sweep                   & -8.89 (39.33\%)   & -17.23 (49.94\%)          & -28.24 (58.11\%) \\
        OR-Tools                & -6.42 (0.00\%)    & -11.50 (0.00\%)           & -17.96 (0.00\%) \\
        Neural-Rewriter         & -6.95 (8.48\%)    & -12.83 (11.83\%)          & -19.45 (8.57\%) \\
        Q-net                   & -6.84 (6.59\%)    & -12.33 (7.37\%)           & -19.27 (7.62\%) \\
        MCTS+random             & -7.65 (19.45\%)   & -20.72 (81.08\%)          & -46.34 (160.11\%) \\
        MCTS+distance           & -7.15 (12.01\%)   & -18.91 (65.04\%)          & -44.00 (147.44\%) \\
        \textbf{SOLO}           & \textbf{-6.21 (-3.18\%)} & -11.25 (-1.98\%) & -17.68 (-1.24\%) \\
        \bottomrule
    \end{tabular}
\end{wraptable}
% \ml{adjustments specific to offline settings + results}
For the offline setting, customers and the depot positions are uniformly sampled from the unit square, while the demands are sampled from a discrete uniform distribution $U[1, 10]$.
The results for the offline settings are presented in \autoref{tab:cvrp_static}.
The experiments demonstrate that despite the fact that SOLO was designed to target the online setting, it maintains decent performance also for the static setting.
The savings algorithm achieves slightly better results than SOLO, showing an average $4\%$ gap compared to  $2\%$ in our case. 
As savings is a problem specific heuristic, it is therefore expected to achieve good results on the offline problem.
% \fr{Wouldn't it make sense to include 20s runtime experiments for the offline setting? It's a little strange we run the online setting with 20s timeout despite the fact that we are already the best approach at 10s. At the same time we do not present 20s timeout results for the offline setting even though we are outperformed by a baseline.}
% \ml{I was trying to build the folloiwng line: Dynamic settings is our target, we're ok on static settings, that's enough. So from the space and time consideration, I would not include this}
% \input{static_pms_table}
% \input{static_table}

\newpage

\subsection{Parallel Machine Scheduling}
%We evaluate the described method on several parallel machine scheduling problems.
For the parallel machine scheduling problem we compare SOLO to the following baselines: the weighted shortest processing times first heuristic (WSPT), neural rewriter \cite{chen2019learning}, and the CPOptimizer of IBM ILOG CPLEX Optimization Studio V12.9.0.
% The baselines we compare our method to are a variant of the weighted shortest processing times first heuristic (WSPT), the neural rewriting approach by \cite{chen2019learning} (neural rewriter), and the CPOptimizer of IBM ILOG CPLEX Optimization Studio V12.9.0.
%\footnote{\url{https://www.ibm.com/support/knowledgecenter/en/SSSA5P\_12.9.0/ilog.odms.studio.help/Optimization_Studio/topics/COS_home.html}} (CPLEX).
See \autoref{app:baselines}.
We also analyze the contributions of our Q-net model and the MCTS component to the overall performance of SOLO by showing Q-net performance with and without MCTS, and by replacing the Q-net model with WSPT in MCTS (MCTS+WSPT). 
We used the same training time for the Q-net and neural rewriter for all problem sizes.
We give MCTS and CPLEX $10$ seconds to optimize each decision.
For additional details please see \autoref{app:training}.

\paragraph{Online Scheduling} 
\begin{figure}[t]
    \centering
    \subfloat[online scheduling 3 machines]{%
        \includegraphics[trim=0 20 0 0, width=0.5\columnwidth]{plots/dynamic-m3.png}
        \label{fig:scheduling-static}
    }
    \subfloat[online scheduling 10 machines]{%
        \includegraphics[trim=0 20 0 0, width=0.5\columnwidth]{plots/dynamic-m10.png}
        \label{fig:scheduling-dynamic}
    }
    \smallcaption{Results for the online PMS benchmark setting on 50 instances each. Lower values indicate better performance. For each approach $a$ and instance $i$, the plot shows the relative disadvantage to CPLEX calculated as $\mathrm{mean}_i((v_a(i) - v_\mathrm{CPLEX}(i)) / v_\mathrm{CPLEX}(i))$.}
    \label{fig:scheduling}
    \vspace{-1.5em}
\end{figure}
We define two online settings, both with $80$ jobs in expectation and $5$ job classes. 
In the first one the jobs that arrive in $16$ intervals of length $130$ time units each have to be scheduled on $3$ machines.
In the second one we use $10$ machines and $60$ intervals of duration $10$. We sample job processing times from $U[1, 100]$, setup times from $U[1, 50]$, and job weights from $U[1, 10]$.
Jobs arrive according to Poisson distributions, where the frequency of the $i$-th class is proportional to $1/i$. 
The problem parameters were chosen as to not overload the machines in steady state on the one hand, while maintaining relatively low levels of idleness.
% We train a Q-net model and evaluate its performance with $50$ random seeds.
Similar to the CVRP setting we run MCTS with a truncated horizon that limits the number of arriving jobs.
%We also used the same training time for the Q-net and neural rewriter for all problem sizes.
As neural rewriter and CPLEX are intended for offline settings, we let them recompute schedules for every decision.

The results are depicted in Figure \ref{fig:scheduling}. 
Q-net outperforms WSPT on average, and is thus a good choice when the time per step is limited. 
When compute time becomes available, MCTS significantly improves the solution.
%\chr{if we want to leave this sentence here i think we need to write a bit more, clearly adding time to MCTS will bring better results} \fr{We're contrasting MCTS@10s with pure G graphnet alone}
In particular, it consistently outperforms WSPT in all problem instances (see \autoref{app:evaluations}). 
Our approach performs mostly on par with CPLEX, with slight advantages for either on different instances. 
neural rewriter generally improves upon WSPT, but does not reach Q-net performance.

\paragraph{Offline Scheduling}
\begin{wraptable}[11]{r}{.45\textwidth}
    % \vspace*{-\baselineskip}
    \vspace{-1.3em}
    \smallcaption{Relative advantage to CPLEX for offline PMS problems on $50$ random instances. Lower values indicate better performance.}
    \label{tab:pms_static}
    \tiny
    \centering
    \begin{tabular}{l*2c}
        \toprule
        baseline & Liao 20 & Liao 80  \\ 
        \midrule
        WSPT                & -16570.16 (5.84\%)          & -182357.02 (4.15\%)         \\
        CPLEX               & -15658.46 (0.00\%)          & -175084.88 (0.00\%)         \\
        Neural-Rewriter     & -16540.28 (5.64\%)          & -182450.02 (4.20\%)         \\
        MCTS+WSPT           & -15876.88 (1.42\%)          & -176439.74 (0.74\%)         \\
        Q-net               & -15906.32 (1.57\%)          & -178444.74 (1.95\%)         \\
        \textbf{SOLO}       & -15695.94 (0.25\%)          & -175524.34 (0.24\%)         \\
        \textbf{SOLO+Prune} & -15683.46 (0.20\%)          & -175164.58 (0.05\%)         \\
        optimal             & -15628.68 (-0.17\%)         & \multicolumn{1}{c}{-}       \\
        \bottomrule
    \end{tabular}
\end{wraptable}
% For the offline setting we consider two benchmark problems: Liao 20 and Liao 80 \cite{Liao2012}.
% In the offline setting the set of jobs is completely known at the first observation.
% First, we consider the offline version of the scheduling problem where the set of jobs is completely known, and for which our baselines were designed. We consider a case with $80$ jobs, $3$ machines, and $5$ job classes.
% A given current state is represented as a bipartite graph of job and machine nodes, where the job and machine features are represented as node features, and edges are labeled with setup times. See \autoref{app:training} for details.
%\ml{maybe we should skip this sentence completely and refer reader to the appendix immediately?} \fr{I would argue against that. We need to give at least a minimal explanation otherwise the paper would no be self-contained.}
For the offline setting we train a model using the same job feature ranges.
%\ml{square brackets are confusing with citations} \fr{square brackets are also common notation for intervals. I think it's unambiguous since you normally have whitespace before a citation.}
We then evaluate it on a public set of benchmark problems that uses the same ranges for job features \cite{Liao2012}.
% \jo{The following sentence introduces more questions. If it wasn't trained on the problems in the benchmark, then what was it trained on?} \fr{I reordered the section to present the offline setting first. For that, I also put the sentence that explains the job feature ranges here. That should answer the questions.}
% The baselines we compare our method to are a variant of the weighted shortest processing times first heuristic (WSPT), the neural rewriting approach by \cite{chen2019learning} (neural rewriter), and the CPOptimizer of IBM ILOG CPLEX Optimization Studio V12.9.0.
%\footnote{\url{https://www.ibm.com/support/knowledgecenter/en/SSSA5P\_12.9.0/ilog.odms.studio.help/Optimization_Studio/topics/COS_home.html}} (CPLEX).
% More details about the baselines can be found in \autoref{app:baselines}.
% We also analyze the contributions of our Q-net model and the MCTS component to the overall performance of SOLO by showing Q-net performance with and without MCTS, and by replacing the Q-net model with WSPT in MCTS (MCTS+WSPT). In all cases, we give MCTS $10$ seconds to optimize each decision.
\autoref{tab:pms_static} shows that although our approach does not specifically target offline problems, it is on par with the optimized baseline CPLEX in this challenging case, indicating that similarly specialized code would have the potential to outperform even CPLEX.
Similar to CVRP, despite the significant growth of problem complexity, we get satisfactory performance for SOLO with fixed training and search time on bigger problems. 
%, showing that it does not sacrifice quality on static problems \jo{static or dynamic?} in favor of performance in dynamic cases. \fr{removed this half-sentence because it no longer makes sense to put here.}
More results are shown in \autoref{app:evaluations}.


==> execution_time.tex <==
\begin{table}[t]
    \caption{Worst-case execution time of SOLO in seconds.}
    \label{tab:execution_time}
    \centering
    \small
    % \begin{sc}
    \begin{tabular}{ll}
        \toprule
        % \multirow{2}{*}{Setting} & \multicolumn{2}{c}{PMS} & \multicolumn{2}{c}{CVRP} \\ % & \textsc{Message-passing} & \textsc{Decoder} & \textsc{N-passes}  \\ 
        Problem & \multicolumn{1}{c}{Execution time [s]} \\
        \midrule
        CVRP Offline size $20$  & $200$ \\ 
        CVRP Offline size $50$  & $500$ \\
        CVRP Offline size $100$ & $1000$ \\[5pt]
        \hline \\[-3pt]
        CVRP Online size $20$   & $5$ & \multirow{3}{*}{\shortstack[l]{Chana, please insert \\ your specs here}} \\ 
        CVRP Online size $50$   & $20$ \\
        CVRP Online size $100$  & $10$ \\[5pt]
        \hline \\[-3pt]
        PMS Offline size $20$   & $14.3$ & \multirow{4}{*}{\shortstack[l]{$18$-core Intel Xeon Gold $6150$ @ $2.70$ GHz \\ Nvidia Tesla V$100$ ($16$ GB)}}\\
        PMS Offline size $80$   & $21.83$ \\
        PMS Online $3$ machines & $6.9$ \\
        PMS Online $10$ machines& $10.65$ \\
        \bottomrule
    \end{tabular}{}
    % \end{sc}
\end{table}
% ($3.70$ GHz max. Turbo)

==> gaussian_mixture.tex <==
\begin{table}[t]
    \small
    \begin{tabular}{l*5c}
        \multicolumn{1}{l}{Distribution} & \textbf{$\mu$} & \textbf{$\sigma$} & \textbf{$w$} & \textbf{$a$} & \textbf{$b$} \\ \\
        \multirow{2}{*}{position $(x, y)$}  & $(0.25, 0.25)$           & $(0.1, 0.1)$  & $0.5$  & $0$ & $1$  \\
         & $(0.75, 0.75)$   & $(0.1, 0.1)$  & $0.5$  & $0$ & $1$  \\
        \hline \\
        \multirow{2}{*}{time $t$}   & \multicolumn{1}{c}{5}  & \multicolumn{1}{c}{3} & 0.33 & 0 & 40 \\
                                    & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{3} & 0.33 & 0 & 40 \\
                                    & \multicolumn{1}{c}{40} & \multicolumn{1}{c}{3} & 0.33 & 0 & 40 \\
    \end{tabular}{}
    \caption{Truncated Gaussian components of Mixture Model distribution for the Online CVRP. $\mu, \sigma, \omega, a$ and $b$ stand for mean, standard deviation, weight, minimum value and maximum value of each truncated Gaussian distribution correspondingly.} \label{tab:online_distribution}
\end{table}
% ($3.70$ GHz max. Turbo)

% \begin{table}[t]
% \centering

% \begin{tabular}{clllll}
% \multicolumn{1}{l}{\textbf{}} & \textbf{$\mu$}           & \textbf{$\sigma$}        & \textbf{$w$} & \textbf{$a$} & \textbf{$b$} \\
% \multirow{}{}{\textbf{position $(x, y)$}} & (0.25, 0.25)           & (0.1, 0.1)            & 0.5  & 0 & 1  \\
%                                  & (0.75, 0.75)           & (0.1, 0.1)            & 0.5  & 0 & 1  \\ 
% \multirow{}{}{\textbf{time $t$}}   & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{3} & 0.33       & 0          & 40         \\
%                                  & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{3} & 0.33 & 0 & 40 \\
%                                  & \multicolumn{1}{c}{40} & \multicolumn{1}{c}{3} & 0.33 & 0 & 40 \\ \hline
% \end{tabular}
% \caption{gaussian mixture distribution for the online VRP }
% \label{tab:online_distribution}
% \end{table}

==> method.tex <==
\section{Method}\label{sec:method}
In the following section we present our method SOLO: Search Online, Learn Offline. An overview of SOLO is depicted in \autoref{fig:methodPlot}. Both the offline and online components are described in detail below.
%In the following section we present our method SOLO: Search Online, Learn Offline where we begin with an offline part description (based on DQN and GNN) and show how it can be used in an online settings (using MCTS). 
%\ml{I guess there's some misconception, MCTS + Q-Net is the online part of SOLO and it can be used in both: offline CO problems and online CO problems. is it correct?}
%\fr{Yes Maksym, that's correct. I would propose to use something like "... where we begin with a description of the offline training part (based on DQN and GNN) and then describe the online search part (using MCTS).} 
%\ml{MCTS is online, no?}



We model the CO problem as a finite horizon Markov Decision Process (MDP;  \cite{puterman1994markov}) of $N$ steps, with states $s$, actions $a$, immediate reward $r(s,a)$, a transition probability $p(s'|s,a)$, and a discount factor $\gamma$. The actions in each step are chosen by a policy $\pi(a|s)$, leading to a state distribution $p(s_N)= p(s_0) \prod_{i=0}^{N-1}\pi(a_i|s_i)p(s_{i+1}|s_i,a_i)$.
The $Q$-function is defined as
\begin{equation*}
    Q(s, a) \triangleq \mathbb{E}_{s'\sim p(s')}\left[\left. \sum_{i=0}^{N} \gamma^i r(s_i,a_i)\right|s_0=s, a_0=a\right],
\end{equation*}
where the agent's objective is to find an  optimal policy  $\pi^*(a|s)= \arg \max_a Q(s,a)$ \cite{sutton2018reinforcement, bertsekas2005dynamic}. 

\paragraph{Learn Offline}
We base our method on 
the  off-policy DQN algorithm where we learn a neural approximation $\tilde{Q}(s,a;\theta) \approx Q(s, a)$ parametrized by $\theta$ \cite{mnih2013playing}. 
%This approximation is trained to minimize the squared temporal difference denoted by $TD$:
%Our goal is to train the network in order to minimize the squared temporal difference (TD) error, denoted by $TD$, which is rearranging of the Bellman Equation \eqref{eq:BE}, i.e.,
%\begin{equation}
%    TD \triangleq r(s, a) + \gamma \max_{s'} %\tilde{Q}(s',a'; \Theta)) - \tilde{Q}(s, a; \Theta),
%\end{equation}
%as is derived from the Bellman Equation. \cd{\cite{.} %needs a reference}
%\fr{remove TD}
%\fr{previous paragraph: Chana and Dotan will edit it}
%
%To address the problem described in the previous section we propose a combined approach where a Q network that was trained offline is used as a search heuristic in MCTS during the online scheduling. \fr{The previous sentence repeats much of what we say in the introduction. Can we focus on the Q network part here?}
%\fr{GNNs are already mentioned earlier in the paper. We should introduce the abbreviation in the introduction. We should also make sure we use a consistent name for GNNs, currently they are sometimes called graph convolutional networks (see related work), sometimes graph neural network (introduction)}
%
% \fr{following paragraph: Maksym will edit it}
% \fr{how do we apply GNNs for modeling the q function? Take material from appendix B}
% \fr{state GNN properties more mathematically: message passing structure; equivariance}
% \fr{put in mathematical terms how our approach differs from related work}
\begin{wrapfigure}[32]{R}{0.4\textwidth}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/SOLO_plot_v05.png}
    \smallcaption{Overview of SOLO. In offline, DQN is used to train a GNN to estimate the Q-value. In online, the estimated Q-value is used in a search for a decision in the current state.}
    \label{fig:methodPlot}
\end{wrapfigure}
Modelling $\tilde{Q}$ using feed-forward or convolutional neural network architectures is challenging in the CO setting as the sizes of the state and action spaces can vary throughout an episode, as the solution to the problem is constructed.
We thus encode a state-action tuple as a graph $G = (w, V, E)$ with the sets of nodes $V$, edges $E$, and global information $w$, and model $\tilde{Q}$ using a Graph Neural Network (GNN).
% Encoding the state-action space as a graph $G = (w, V, E)$ with the sets of nodes $V$, edges $E$ and global information $w$, however, yields a size invariant representation.
This lets us address the changing size of a problem (i.e., different $|V|$ and $|E|$ per step) in a principled manner.
% In order to operate on the graph representation of the input space we model $\tilde{Q}$ using a Graph Neural Network (GNN).
We use a variant of the massage-passing GNN architecture \cite{battaglia2018relational} with update rules
\begin{equation*}
    \begin{split}
        e_i^{(t+1)} & = \phi_e(e_i^{(t)}, \rho^{v\to e}(V), w), \forall e_i \in E,\\
        v_i^{(t+1)} & = \phi_v(v_i^{(t)}, \rho^{(e, v)\to v}(V, E), w), \forall v_i \in V,\\
        w^{(t+1)} & = \phi_w(w^{(t)}, \rho^{(e, v)\to w}(V, E)),
    \end{split}
\end{equation*}
where $\rho^{v\to e}$, $\rho^{(e, v)\to v}$, $\rho^{(e, v)\to w}$ are the aggregation functions that collect information from the \textit{related} parts of $G$, and $\phi_e$, $\phi_v$, $\phi_w$ are the neural networks that update the feature vectors $e_i \in E$, $v_i \in V$ and $w$, respectively.
% \fr{neighbouring instead of related?} \ml{not true for global information} 
% Message passing consist of two steps that are applied repetitively: information aggregation and feature update.
% During the information aggregation step feature vectors of $V$, $E$ and $w$ are concatenated with the information from the \textit{related} entities of the $G$ aggregated by the function $\rho$.
% Related entities of the graph are adjacent nodes for the $V$, sending and receiving nodes for $E$ and the complete set of $E$ and $V$ for the $w$.
% Aggregated information is then passed to one of three neural networks $\phi_e$, $\phi_v$ and $\phi_g$ .
% The final update rule for the edge information is $e_i^{t+1} = \phi_e(e_i^t, \rho^{v\to e}(E), w)$
% \begin{equation*}
%     v_i^{t+1} = \phi_v(v_i^t, \rho^{e\to v}(v_j), w)
% \end{equation*}
% \ml{too long :(}
% \ml{extend above sentence}
We compute $\tilde{Q}(s, a)$ as the the output of $\phi_e$ at the final message-passing step.
% That allows for the action space of the varying size for every observation as 
The resulting GNN architecture is equivariant, meaning that for some permutational transformation $T$ the following property holds: $T(\tilde{Q}(s, a)) = \tilde{Q}(T(s, a))$.
Additionally, it explicitly represents the action space of varying size.
That allows us to leverage the fact that creating partial solutions induces smaller subproblems that correspond to smaller input graphs, and use these as the encodings for the successor states.
For more details on architecture see \autoref{app:training}.
% \fr{Would it require much space to make the encoder->message passing->decoder architecture explicit?}
% \ml{depends: if completely explicit - you'll need to introduce 6 more networks, right? maybe we can refernce to abstract?}
% Additionally, due to the properties of GNN, it does natively support the actions space of varying size. \ml{taht was mentined above}

% Contrarily to fixing the action space with a fully connected final layer \cite{MaoEtAl2019,Mao2016} or masking nodes that are already part of a partial solution \cite{KhalilEtAlNIPS2017,Kool2019ICLR}.
% We propose to leverage the fact that creating partial solutions induces smaller remaining subproblems that correspond to smaller input graphs, and use these as the encoding for the successor states.
% This makes masking unnecessary and also enables us to apply our approach to problems where the graph can \textit{grow} over the course of an episode, even beyond the problem size in the initial state.
% Graph Neural Networks (GNN)s allow learning of neural networks on graph input spaces.


% GNNs are permutation equivariant \cite{zaheer2017deep} and are able to process observations of varying sizes (i.e., different number of nodes and edges) as long as features dimensionality remains constant. 
% In addition, GNNs are able to leverage the relational bias in observations via multi-step propagation of information within the graph representation, i.e., message-passing \cite{hamrick2018relational}.
% \cd{Can we add one or two sentences on the GENERAL insights on how to model the space as a graph here?}
% \ml{I will add ref to the appendix, where it's described precisely}
% Instead of using masking or fixing the actions space with the fully connected layer (see \autoref{sec:related_work}) 
% \fr{I find it awkward to have this point distributed between here and the related work section. Now you need to (1) explain parts of our approach in the related work section, instead of the method section where you can explain it properly, and (2) you cannot be specific about what related work you mean here. I much prefer having the exact references here. It would also serve Chris' comment about describing challenges we had to overcome to make our approach work in the method section.}, we propose to exploit the fact that creating partial solutions induces smaller remaining subproblems that correspond to smaller input graphs.
%, and use these as successor states.
% Using these sub-graphs as successor states makes masking unnecessary and furthermore enables us to apply our approach to problems where the graph can \textit{grow} over the course of an episode, even beyond the problem size in the initial state.
% Additionally this method implicitly includes the information about the eligibility of actions into the training procedure.
% For the set of problems where graph representation alone cannot encode the eligibility of an action this information can be included to the input features of the graph and addressed during the learning in a principled manner (see \autoref{app:training}).

% GNNs repetitively apply a set of neural networks to the graph representation of the input data $G = (w, U, V, E)$ \fr{@Maksym: it's not clear what $(w, U, V, E)$ are}\dd{Indeed}.
% GNNs have several properties that are important in the context of combinatorial optimization:
% They are permutation equivariant \cite{zaheer2017deep} and are able to process observations of varying sizes (i. e., different number of nodes $V$ and edges $E$) as long as features dimensionality remains constant. 
% In addition, GNNs are able to leverage the relational bias in observations via multi-step propagation of information within the graph representation, i.e., message-passing \cite{hamrick2018relational}.

% in an invariant manner, however, is possible by  
% To learn a policy on the graph representation, we model $\tilde{Q}$ using a Graph Convolutional Neural Network (GCN). \cd{what are the interesting propoerties of a convolutional GNN?}
% We employ Graph Neural Networks (GNN) as a $\tilde{Q}$ function approximator in our DQN algorithm implementation.

% \jo{Much of this discussion should probably be moved to the related work section.} 
% \fr{I would agree with Chris and Maksym that these more detailed comparisons should be here. For some, the context of our method is required to understand the differences. For others, shortcomings of existing work motivate our approach.}
% The combination of GNNS and RL has recently been exploited to solve combinatorial optimization problems \cite{KhalilEtAlNIPS2017,Kool2019ICLR,MaoEtAl2019,Mao2016}.
% by leveraging the relational bias and information propagation within the graph structure.
% We also follow that approach and compute $Q$ values as the updated features of edges $E$ or nodes $V$ after the application of GNN. 
% A notable difference, however, is how we treat the changing dimensionality of the state and action space throughout an episode:
% Existing work either fixes the action space with a fully connected final layer \cite{MaoEtAl2019,Mao2016} or addresses this challenge by masking nodes that are already part of a partial solution \cite{KhalilEtAlNIPS2017,Kool2019ICLR}.
% Instead, we propose to leverage the fact that creating partial solutions induces smaller remaining subproblems that correspond to smaller input graphs, and use these as successor states.
% This makes masking unnecessary and also enables us to apply our approach to problems where the graph can \textit{grow} over the course of an episode, even beyond the problem size in the initial state.
%\ml{what about small rearrangement?: The combination of GNNS and RL has recently been exploited to solve combinatorial optimization problems \cite{KhalilEtAlNIPS2017,Kool2019ICLR,MaoEtAl2019,Mao2016}.
%by leveraging the relational bias and information propagation within the graph structure.
%A notable difference, however, is how we treat the changing dimensionality of the state and action space throughout an episode:
%Existing work either fixes the action space with a fully connected final layer \cite{MaoEtAl2019,Mao2016} or addresses this challenge by masking nodes that are already part of a partial solution \cite{KhalilEtAlNIPS2017,Kool2019ICLR}.
%Instead, we propose to leverage the fact that creating partial solutions induces smaller remaining subproblems that correspond to smaller input graphs, and use these as successor states.
%We compute $Q$ values as the updated features of edges $E$ or nodes $V$ after the application of GNN. (I guess here something is missing that's why you want to put the at the beginning, since others also might put the $Q$ values to the nodes or edges). 
%This makes masking unnecessary and also enables us to apply our approach to problems where the graph can \textit{grow} over the course of an episode, even beyond the problem size in the initial state.
%and the last point: Additionally this method implicitly includes the information about the eligibility of actions into the training procedure.
%}
%\ml{1) there's a bit of repetition of last sentence of the previous paragraph. Do you propose to delete it? 2) the sentence which begins with "this makes masking unnecessary", now there's no explanation of why it's unnecessary. Previously it was connected with the fact that GNN can handle varying number of nodes and edges. Maybe we could insert intermediate sentence with something like "We're proposing to achieve that by compute the $Q$ values as the updated features of edges $E$ or nodes $V$ after the application of GNN" ? }
% Combination of GNN and RL is not novel and was recently applied to the combinatorial optimization.
% However, to the best of our knowledge, GNNs were used to exploit the relational bias and facilitate the information propagation within the graph structure. 
% Whereas the changing dimensionality of online combinatorial problems was addressed by masking approaches \ml{citations}.
% By contrast, in our method we propose to compute the $Q$ values as the updated features of edges $E$ or nodes $V$ after the application of GNN.
% This approach allows to have the estimate of $Q$ value for the varying number of actions at different observation of MDP and eliminates the necessity of masking.
% That significantly shrinks the action space, which might be the concern for the problems of bigger size, as well as implicitly includes the information about the eligibility of actions into the training procedure.
% Additionally this method implicitly includes the information about the eligibility of actions into the training procedure.
% For the set of problems where graph representation alone cannot encode the eligibility of an action this information can be included to the input features of the graph and addressed during the learning in a principled manner (see \autoref{app:training}).


% The graph structure is the only part of the method that is particular to the problem and has to be redefined depending on application.

% For the scheduling problem, we represent each observation with a bipartite, undirected graph represented by the tuple $G = (w, U, V, E)$.
% In the proposed encoding $U = \{u_i\}_{i=1:N_u}$ and $V = \{v_j\}_{j=1:N_v}$ correspond to two disjoint independent sets of nodes, where $u_i$ is the feature vector of machine $i$ and $v_j$ the feature vector of job $j$.
% The machine and job feature vectors consist of the characteristics described in \autoref{sec:problem}.
% For implementation reasons, the actual feature vector of every node $u_i \in U$ and $v_j \in V$ is the concatenation of machine and job features where the irrelevant dimensions are masked by zeros.
% The sets of machine and job nodes are interconnected by the set of edges $E = \{(e_k, m_k, j_k)\}_{k=1:N_e}$, where $e_k$ is a edge feature vector, $m_k$ is an index of a machine node, and $j_k$ an index of a job node connected by the edge $k$.
% Edge features encode the setup time required to process the job $j_k$ on corresponding machine $m_k$.
% Additionally, the graph representation contains $w$ that is the global information vector relevant for the entire graph.
% In the current implementation $w$ is initialized to 0 for every observation, however it is used for the information propagation during the message-passing.

% We use the encoding message-passing decoding GNN architecture as described by \cite{battaglia2018relational}.
% In the encoder part, the edge network $\phi_e$, node network $\phi_n$, and global network $\phi_g$ are implemented as one fully connected layer followed by layer normalisation.
% In the message-passing part, each of the three networks consists of three fully connected layers and layer normalization after the last fully connected layer.
% Additionally, for the node network $\phi_n$, a multi-head self-attention mechanism \cite{Kool2019ICLR} was implemented on top of the message-passing architecture.
% The Decoder networks consist of one, fully connected layer each.
% The total number of trainable parameters for the GNN architecture is provided in \autoref{tab:totalParams}.
% Given the bipartite structure of our graph $2$ message-passes are enough to cover the longest path.

% The result of the GNN application is a graph of the same structure but with the updated nodes $u_i$ and $v_j$, edge $e_k$ and global $w$ feature vectors.
% Feature $e_k$ of edge $k$ is interpreted as the Q-value of scheduling job $j_k$ on machine $m_k$ and global feature $w$ as the Q-value of \texttt{noop} action.

% Our DQN implementation includes various improvements that were suggested by \cite{hessel2018rainbow} such as dueling, double Q, delayed target network updates, prioritized replay and multi-step reward estimation.
%From our experience, the training performance was not very sensitive to the described DQN improvements. \ml{note: didn't experiment with delayed target network update}
% In order to optimize the model and to train its parameters, including the number of message-passes, we applied a hyperparameter search algorithm that is based on successive halving \cite{kumar2018parallel}.


% Monte-Carlo Tree Search (MCTS) is a powerful online planning method for sequential and (possibly) stochastic decision problems. 
% Briefly, MCTS operates by searching for the optimal decision to make at each state via iteratively sampling rollouts: sequences of steps that begin in the current state and end in either terminal states or states that were reached by the end of the planning horizon. 
% These rollouts are used to build a search tree, which stores information about the visited states. Such information includes Q-value estimations $Q^{\mathcal{T}}\left(s,a\right)$ that are used to guide the search in subsequent rollouts and eventually, when timeout is reached, output a decision for the current state. 
% MCTS serves as a core mechanism in several success stories, e.g., .
% While MCTS is capable of finding high-quality decisions without incorporating any domain-specific knowledge \cite{silver2017mastering}, the availability of good domain-specific heuristics can significantly facilitate the search process, yielding better decisions in shorter deliberation times.

% previous version: One of the major challenges of combintorail optimization is the significant impairing influence of sub-optimal actions during the computation of partial solution on the final performance} \ml{please help me rephrase that}
% Next, we need to address the challenge that in an NP-hard problem, the question of whether a single action is optimal is also NP-hard\footnote{Otherwise one could solve an NP-hard problem of size $N$ by combining $N$ non-NP-hard optimal decisions, which would not be NP-hard.}. In particular, making the wrong choice can severely impact the final solution quality. \dd{AFAIK, you cannot start a sentence with E.g. Instead,
% "For example,"}E.g., for the bin packing problem, no polynomial time algorithm can produce solutions guaranteed to be better than $\frac{3}{2}$ of the optimal solution value unless P = NP \cite{vazirani2013approximation}.

\paragraph{Search Online}
We use online search to optimize the decisions in the states observed in real time. Namely, we take the time until the next decision is due (e.g., next job assignment or next customer pick-up) to evaluate all the applicable actions in the current state and, when reaching the timeout, output the estimated best action for this state.

For this purpose, we employ a popular MCTS algorithm called UCT (Upper Confidence-Bound applied to Trees) \cite{kocsis2006bandit} in conjunction with the Q-value estimate $\tilde{Q}(s, a; \Theta)$ (henceforth $\tilde{Q}$-value) trained offline. More specifically, we iteratively sample rollouts from the (current) root state until a terminal state by sequentially choosing actions according to the Upper Confidence-Bound (UCB) policy \cite{kocsis2006bandit} and estimate the Q-Value of the encountered states $s$ and actions $a$ as $Q^{\mathcal{T}}\left(s,a\right)=\sum_{i=1}^{n_{s,a}}  \frac{\overline{r}_i}{n_{s,a}}$, where $\overline{r}_i$ is the sample (rollout) $i$ accumulated reward from state $s$ until the end of the rollout. UCB balances exploration and exploitation by choosing an action that was not yet sampled if such action exists, and otherwise it chooses the action that maximizes the value $Q^{\mathcal{T}}\left(s,a\right) + \beta\sqrt{\frac{\log\left(n_s\right)}{n_{s,a}}}$, with $n_{s,a}$ denoting the number of times action $a$ was sampled in state $s$, $n_s=\sum_{a}n_{s,a}$, and $\beta$ is the exploration factor.

While UCT is guaranteed to asymptotically converge at the optimal decision by sampling each action infinitely often, in order to improve its practical efficiency, we combine it with our trained network in a twofold manner:
First,  we use the $\tilde{Q}$-value as an out-of-tree heuristic. We employ an iterative deepening scheme according to which, in each iteration, the search tree is expanded with at most one state, which is the first state in the rollout that is not already in. During rollout, when we encounter states that are not yet in the tree, we choose the action that maximizes the $\tilde{Q}$-value rather than using UCB (corresponding to a random action in this case). This is a common technique that often improves performance significantly, depending on the quality of the used heuristic.
Second, we use the $\tilde{Q}$-values to prune the action space. Since the number of plausible actions in CO problems tends to be intractably high, we would like to focus the samples on actions that have higher potential to be a (near-)optimal action. We thus consider for each state $s$ only the $k$ actions with the highest $\tilde{Q}$-value, where $k$ is a hyper-parameter of our algorithm. Indeed, as the estimated $\tilde{Q}$-value becomes more accurate, the probability that one of these $k$ actions is near-optimal increases.
In addition, in order to allow more samples for the considered actions, we shorten the lookout period by terminating a rollout before the end of the horizon, having the termination criteria dependent on the specific problem setting. By applying the above features, we theoretically compromise optimality, but our experiments demonstrate that they hold some practical merits. 

%In combinatorial optimization problems, making sub-optimal choices at the earlier stage of solution computation can have an over-proportionally large effect on the final solution quality.
%\fr{@Maksym I see the part where I elaborated on the over-proportionally large impact mentioned in the previous sentence was removed. Do we think we can get away without explaining this?}
%In order to compensate for this imbalance, we apply UCT \cite{kocsis2006bandit}, a variant of a Monte-Carlo Tree Search (MCTS), in combination with the GCN which was trained offline using DQN.
%Specifically, we sample rollouts by choosing actions according to the Upper Confidence-Bound (UCB) policy \cite{kocsis2006bandit} for states that are inside the search tree (i.e., added to the tree in preceding rollouts), and otherwise choose the action with the highest Q-value estimate $\tilde{Q}(s, a; \Theta)$, obtained from the trained GCN. 
%\ml{Zohar, I'll try to extract your equations from text.. please comment}\zf{Thanks for taking care of this. Looks good}
%UCB balances exploration and exploitation by trying first all actions once, and afterwards choosing the action that maximizes the value $Q^{\mathcal{T}}\left(s,a\right) + \beta\sqrt{\frac{\log\left(n_s\right)}{n_{s,a}}}$, where $n_{s,a}$ denotes the number of times action $a$ was sampled in state $s$, $n_s=\sum_{a}n_{s,a}$, and $\beta$ is the exploration factor. The Q-values in each states are estimated as $Q^{\mathcal{T}}\left(s,a\right)=\sum_{i=1}^{n_{s,a}}  \frac{\overline{r}_i}{n_{s,a}}$, where $\overline{r}_i$ is the sample (rollout) $i$ accumulated reward from state $s$ until the end of the rollout.
%UCB balances exploration and exploitation by trying first all actions once, and afterwards choosing the action that maximizes $Q^{\mathcal{T}}\left(s,a\right) + \beta\sqrt{{\log\left(n_s\right)}/{n_{s,a}}}$,
% \dd{(1) We can make the following equation inline.} \ml{I guess the fraction that is in this equation will look ugly in inline mode}:
% \dd{(2) It doesn't have label, thus, we should use the environment equation* instead of equation}
% \dd{(3) It is not our invention... We should add here reference to be fair and hint the reader that we are stating known result.} \fr{the reference is in the paragraph directly before the equation: \cite{kocsis2006bandit}}
% \begin{equation*}
%     Q^{\mathcal{T}}\left(s,a\right) + \beta\sqrt{\frac{\log\left(n_s\right)}{n_{s,a}}},
% \end{equation*}
%where $n_{s,a}$ denotes the number of times action $a$ was sampled in state $s$, $n_s=\sum_{a}n_{s,a}$, and $\beta$ is the exploration factor. 
%The Q-values in each states are estimated as $Q^{\mathcal{T}}\left(s,a\right)=\sum_{i=1}^{n_{s,a}}  \frac{\overline{r}_i}{n_{s,a}}$, where $\overline{r}_i$ is the sample (rollout) $i$ accumulated reward from state $s$ until the end of the rollout.
%The Q-values in each states are estimated as
%\begin{equation*}
%    Q^{\mathcal{T}}\left(s,a\right)=\sum_{i=1}^{n_{s,a}}  \frac{\overline{r}_i}{n_{s,a}},
%\end{equation*}
%where $\overline{r}_i$ is the sample (rollout) $i$ accumulated reward from state $s$ until the end of the rollout.
%Note in particular that choosing UCB results in an anytime-optimal algorithm, i.e., one that converges to the optimal solution of the online combinatorial problem.
%\ml{I would formulate this similar to line 66: by contrast with Method 1, Method 2 (ref ot related work), UCB ...}
%Sampling multiple rollouts using the GNN and taking the best action \cite{Kool2019ICLR} does not offer the same guarantee. 
%The randomized breadth-first search used by \cite{Zhuwen2018} is also not applicable since it only keeps tracks of partial solutions and does not represent the probability of sampling the corresponding problem realizations.
%\chr{im not sure i would have this here, its again a comparison to other methods, no?}

%Furthermore, we employ an incremental deepening scheme according to which, in each iteration, the search tree is expanded with at most one state, which is the first state in the rollout that is not already in.
%Since the number of actions in some cases can be quite large, often leading to poor performance, we consider a pruning mechanism that makes use of the GNN in additional manner. Namely, during search, we consider only the $k$ actions with the highest Q-values estimates $\tilde{Q}(s, a; \Theta)$.
%Online part of SOLO is presented on \autoref{fig:method-plot}.
%\fr{@Maksym There is no still introduction of the rollout truncation here, in contrast to what was planned in the commented-out parts below. Was there a conscious decision against explaining it here? I would argue we should introduce it here, since is used in both scheduling and CVRP.}
%https://www.overleaf.com/6433478889yhbrcfftnfdc
% \ml{Here goes difference to existing approaches.} \fr{I don't think we need more here: The properties of our MCTS algorithm are fully describe above. Other work on combining ML and combinatorial optimization does not use MCTS.}
% The overall architecture of the proposed method is presented in \autoref{fig:method-plot}.
% \fr{a description of the rollout truncation technique is still missing here.}

% \dd{What is most missing here (and I know the spacex problem) is that we do not have any algorithm, or the least, some paragraph that states "Our Method" (!) \\
% I would split the method with subsections.\\
% A suggestion: \\
% 3.1 DQN \\
% 3.2 MCTS, \\
% 3.3 Our method.\\
% Alternatively, we can  have the full blown Algorithm environment (which is pricey in space).\\
% Also, we do not need to use subsection but we can just have inline bold subsections...\\
% }\chr{i agree and think we should revise this whole part. also in MCTS we should add that we used truncated rollouts in the online problems - this allows for more rollouts in a given timeout and also allows the algorithm to have a balance between future rewards and current actions}
% \fr{If our goal is to define what our method is, then would it not be enough to finish the section with a recap like this? "SOLO is the combination of the components described above, i.e., a GNN trained offline with DQN, which is online used within a specialized MCTS search as a heuristic. The specialized MCTS search employs rollout truncation and optionally action pruning. We denote these cases as SOLO and SOLO+prune, respectively.}

==> model.tex <==
\section{Q Graphnet Model and Training Details}\label{sec:model}

As mentioned, RL has shown to be a promising approach to address the stochasticity of combinatorial problems. We model the problem as a Markov Decision Process (MDP; \cite{puterman1994markov,sutton2018reinforcement, bertsekas2005dynamic}), where $X$ and $A$ are the state and action spaces respectively, and $P(x'|x,a)$ denotes the probability of transitioning from state $x\in X$ to state $x'\in X$ when applying action $a \in A$. 
The agent maintains a policy $\pi_\theta(a|x)$  that expresses the probability to choose an action $a\in A$ given that it is in state $x \in X$. We define a $Q$ function to be     
$Q(x, a) \triangleq \mathrm{E}^{\pi_\theta}\left[\left. \sum_{i=0}^{N} \gamma^i r(x_i,a_i)\right|x_0=x, a_0=a\right]$ where where $\mathrm{E} [\cdot]$ is the expectation w.r.t.\ the transition probabilities and policy, $0 \le \gamma \le 1$ is the \emph{discount factor} and $N$ is the reward-to-go horizon (in our case finite but may be stochastic as well). This function represents the cumulative discounted reward for applying $a$ at $x$ and then following some policy of actions which could be greedy or explorative \cite{sutton2018reinforcement, bertsekas2005dynamic}. The goal of the agent it optimize the $Q$-function by finding the optimal policy $\pi_\theta(\cdot|\cdot)$.

To solve the MDP formulation we use the off-policy DQN algorithm that learns an approximation to $Q(s, a)$. This cumulative discounted reward can be split into the immediate reward, $r(x,a)$, and the policy return $R(x)$, i.e., $Q(x,a) = E[r(x, a) + R(x)| x, a]$
where $R(x)  =  E[\sum_{i = 1}^{N} \gamma^{i} r(x'_{i}, a_{i})|x]$. Rearranging the equation yields the Bellman Equation $Q(x,a) = E[r(x, a) + \max_{a'}Q(x', a')]$.

Due to both the large state space $X$ and the $Q$ function complexity, a neural network parametrized by $\Theta$ is a common choice for $Q$ function approximation.
%Commonly, due to the large state space $S$ and complexity of the t a neural network function approximation parametrized by $\Theta$ is used to approximate $Q$ function to address both large state space $S$ and the complexity of approximated function.
%\fr{We use a neural function approximation to address both large state space $S$ and the complexity of approximated function.}
%\zf{$Q^{\mathcal{N}}$ (align with forward notation I use in MCTS} in order to approximate the Q-value $Q(s,a)$ where we parametrize it using $\Theta$.
%\ml{Somehow the above sentense sounds too overcomplicated. How about that: "$Q$ function approximation parametrized by $\Theta$ is trained to minimize the temporal difference (TD) error"? The fact that approximation is Neural net is addressed in following paragraph.}
This approximation is trained to minimize the squared temporal difference denoted by $TD$, which is derived from the Bellman Equation, i.e.,
%Our goal is to train the network in order to minimize the squared temporal difference (TD) error, denoted by $TD$, which is rearranging of the Bellman Equation \eqref{eq:BE}, i.e.,
%\begin{equation*}
$ TD \triangleq r(x, a) + \gamma \max_{x'} Q(x',a'; \Theta)) - Q(x, a; \Theta)$.
%\end{equation*}

%To address the problem described in the previous section we propose a combined approach where a Q network that was trained offline is used as a search heuristic in MCTS during the online scheduling. \fr{The previous sentence repeats much of what we say in the introduction. Can we focus on the Q network part here?}
%\fr{GNNs are already mentioned earlier in the paper. We should introduce the abbreviation in the introduction. We should also make sure we use a consistent name for GNNs, currently they are sometimes called graph convolutional networks (see related work), sometimes graph neural network (introduction)}
We employ GNN as a $Q$ function approximation in our DQN algorithm implementation.
GNN is a common name for the framework where a set of neural networks is repetitively applied to the graph representation of the input data.
GNNs have several properties that are important in a context of combinatorial optimization:
They are permutation equivariant \cite{zaheer2017deep} and are able to process observations of varying sizes (i. e., different number of nodes and edges) as long as features dimensionality remains constant. 
In addition, GNNs are able to leverage the relational bias in observations via multi-step propagation of information within the graph representation, i.e., message-passing \cite{hamrick2018relational}.

The graph structure is the only part of our method that is particular to the problem and has to be redefined depending on application.
For the scheduling problem, we represent each observation with a bipartite, undirected graph represented by the tuple $G = (w, U, V, E)$.
In the proposed encoding $U = \{u_i\}_{i=1:N_u}$ and $V = \{v_j\}_{j=1:N_v}$ correspond to two disjoint independent sets of nodes, where $u_i$ is the feature vector of machine $i$ and $v_j$ the feature vector of job $j$.
The machine and job feature vectors consist of the characteristics described in \autoref{sec:problem}.
For implementation reasons, the actual feature vector of every node $u_i \in U$ and $v_j \in V$ is the concatenation of machine and job features where the irrelevant dimensions are masked by zeros.
The sets of machine and job nodes are interconnected by the set of edges $E = \{(e_k, m_k, j_k)\}_{k=1:N_e}$, where $e_k$ is a edge feature vector, $m_k$ is an index of a machine node, and $j_k$ an index of a job node connected by the edge $k$.
Edge features encode the setup time required to process the job $j_k$ on corresponding machine $m_k$.
Additionally, the graph representation contains $w$ that is the global information vector relevant for the entire graph.
In the current implementation $w$ is initialized to 0 for every observation, however it is used for the information propagation during the message-passing.

We use the encoding message-passing decoding GNN architecture as described by \cite{battaglia2018relational}.
In the encoder part, the edge network $\phi_e$, node network $\phi_n$, and global network $\phi_g$ are implemented as one fully connected layer followed by layer normalisation.
In the message-passing part, each of the three networks consists of three fully connected layers and layer normalization after the last fully connected layer.
Additionally, for the node network $\phi_n$, a multi-head self-attention mechanism \cite{Kool2019ICLR} was implemented on top of the message-passing architecture.
The Decoder networks consist of one, fully connected layer each.
The total number of trainable parameters for the GNN architecture is provided in \autoref{tab:totalParams}.
Given the bipartite structure of our graph $2$ message-passes are enough to cover the longest path.

The result of the GNN application is a graph of the same structure but with the updated nodes $u_i$ and $v_j$, edge $e_k$ and global $w$ feature vectors.
Feature $e_k$ of edge $k$ is interpreted as the Q-value of scheduling job $j_k$ on machine $m_k$ and global feature $w$ as the Q-value of \texttt{noop} action.

Our DQN implementation includes various improvements that were suggested by \cite{hessel2018rainbow} such as dueling, double Q, delayed target network updates, prioritized replay and multi-step reward estimation.
%From our experience, the training performance was not very sensitive to the described DQN improvements. \ml{note: didn't experiment with delayed target network update}
In order to optimize the model and to train its parameters, including the number of message-passes, we applied a hyperparameter search algorithm that is based on successive halving \cite{kumar2018parallel}.

\input{parameters_table.tex}

==> parameters_table.tex <==
\begin{table}[t]
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{*6c}
        %\toprule
        \textbf{Problem} & \textbf{Network} & \textbf{Embedding} & \textbf{GNN} & \textbf{Output} & \textbf{N-passes}  \\ 
        %\midrule
        PMS   & $\phi_e$, $\phi_n$ & $32$  & $32 \quad 32 \quad 32$ & $1$  &  \multirow{2}{*}{4} \\ 
        & $\phi_g$ & $32$  & $32 \quad 32 \quad 32$ & $1$  & \\
         CVRP   & $\phi_e$, $\phi_n$ & $256$  & $256 \quad 256 \quad 256$ & $1$  &  2\\
        & $\phi_g$ & $256$  & $256 \quad 256 \quad 256$ & $2$  & \\
    \end{tabular}%
    }
    \caption{Output dimensions of fully connected layers and number of message passes for edge $\phi_e$, node $\phi_n$ and global $\phi_g$ networks}
    \label{tab:totalParams}
\end{table}

==> problem.tex <==
\section{Problem Statements}
\label{sec:problem}
% There are many combinatorial problems in which the underlying tasks are to find the best processing order over a collection of entities. Among them are routing problems like the travelling salesperson problem (TSP) as well as the scheduling problems. In this context, it is natural to consider online variants where additional entities appear at various point during the execution of the algorithm  according to a known distribution. We address two such problems: the parallel machine scheduling problem and the capacitated vehicle routing problem, and their online versions.
The following section introduces offline and online versions of the capacitated vehicle routing problem and parallel machine scheduling.

\subsection{The Capacitated Vehicle Routing Problem}
We consider a simplified version of the Capacitated Vehicle Routing problem (CVRP) introduced by Dantzig and Ramser~\cite{dantzig59}. There is a  set $N = \{ 1,\ldots,n \}$ of customers with individual demands $\{d_i \}_{i=1,\ldots,n}$ for a single commodity, and locations $\{p_i \}_{i=1,\ldots,n}$. The commodity is located at a depot $o$, and is to be transported from it to the customers so as to meet their demand by a vehicle of capacity $C^*$ (for feasibility, we assume that $d_i \leq C^*$ for all $i \in N$). There is a function $c(p, p')$ that prescribes the cost of travelling from location $p$ to location $p'$. A \textit{tour} consists of a path,  $\tau = (p_1 = o, \ldots, p_{n_{\tau}} = o)$, in which the vehicle's load does not exceed its capacity and satisfies the demands of the customers along it. The \textit{cost} of the tour $\tau$ is simply the total cost of travelling from along it: $c(\tau) = \sum_{i=1,\ldots,n_{\tau}-1}c(p_i, p_{i+1})$. A \textit{solution} for the capacitated vehicle routing problem is composed of a sequence of tours $\tau=\tau_1,\ldots,\tau_k$ that covers all the customers. Its \textit{cost} is the sum of its tours $\sum_{i=1,\ldots,k} c(\tau)$. The objective, for a given instance, is to find a solution that minimizes the the total cost while satisfying all the customers' demands\footnote{It is easy to see that CVRP is a generalization of the Travelling Salesperson problem (TSP).}. In our experiments, we consider the Euclidean metric, where the customers locations are located in $\mathbb{R}^2$ and the cost function is simply the $L_2$ distance metric. Furthermore, the vehicle's velocity, which determines the time required to travel from one point to another, is also included in the description of the problem instance.
At every decision point, the agent's set of actions consists of the valid customers (those whose demands do not exceed its remaining capacity and have not yet been satisfied) and the depot (in the event that it is not already there). 
For more details on environment dynamics, refer to Appendix \ref{app:cvrp_dynamics}.
% \fr{for removing the environment dynamics, add this here: At every decision point, the agent's set of actions consists of the valid customers (those whose demands do not exceed its remaining capacity and have not yet been satisfied) and the depot (in the event that it is not already there). For more details on environment dynamics, refer to Appendix \ref{app:dynamics}}

\paragraph{Online CVRP} We
%\chr{now that we moved this to be the first problem should not say again}\fr{thanks Chana, I missed that one}
consider an online version, in which the customers arrive at times sampled from a distribution, while the vehicle is touring along the customers and depot. A decision point occurs when the vehicle arrives at its next target location,  and there is at least one available customer.\footnote{Note that that travel time between customers varies according to the distances between them, and thus one or more customers may arrive during the vehicle's travel.} 

% \paragraph{The environment dynamics} In both variants of the problem, we model the system as an MDP as follows. At every decision point, the agent's set of actions consists of the valid customers (those whose demands do not exceed its remaining capacity and have not yet been satisfied) and the depot (in the event that it is not already there). An observation at time $t$, $\left< N_t, \mathbf{v}_t, C_t \right>$,  comprises the set of available customers $N_t$, including those with demands that exceed the current remaining capacity $C_t$, the vehicle's location $\mathbf{v}_t$, and its remaining capacity $C_t$. Upon the selection of a customer $i$ (or depot) by the agent at time $t$, the immediate reward is the negative distance travelled from the current location to the customer, and the vehicle's capacity is updated to $C_t - d_i$ if the action corresponds to a customer, or the initial capacity $C^*$ if the depot is selected.


\subsection{Parallel Machine Scheduling}

We consider (offline) scheduling problems  \cite{KRAMER2019} where a number of jobs $N = \{ 1,\ldots,n \}$ are to be processed by a set of identical machines $M = \{ 1,\ldots,m \}$. Jobs are characterized by their classes $\{s_i \}_{i=1,\ldots,n}, s_i \in \{1, \dots, s \}$, processing time $\{p_i \}_{i=1,\ldots,n}$, and weights $\{w_i \}_{i=1,\ldots,n}$. Each machine can only process one job at a time and will take $p_i$ time units to complete it. Whenever two jobs $i, j$ are processed consecutively on a single machine, the setup of the machine might need to be changed, which incurs a time penalty (i.e., setup time) of $f(s_i, s_j)$, where $f(s_i, s_i) = 0$. We adopt the total weighted completion time (TWCT) objective, given by $\Gamma(\mathbf{c}) \triangleq \sum_{i \in N} w_i \cdot c_i$ where $c_i$ is the completion time of $i$ (i.e., the time when $i$ has finished processing).
Actions are represented by tuples $(j, m)$, corresponding to processing job $j$ on machine $m$. 
For more details on environment dynamics, refer to Appendix \ref{app:pms_dynamics}.
% \fr{for removing the environment dynamics, add this here: Actions are represented by tuples $(j, m)$, corresponding to processing job $j$ on machine $m$. For more details on environment dynamics, refer to Appendix \ref{app:dynamics}}

\paragraph{Online Parallel Machine Scheduling}
%While all relevant jobs are visible in the initial state in offline settings, 
Additional jobs can arrive at a finite number of points in time (arrival intervals) in the online settings. The number of arriving jobs at the start of each interval is determined by an arrival distribution for each class (e.g., Poisson).

%\zf{is it clear at this point that we use a simulator and why? if not, it's worth saying a few words}
% \paragraph{The environment dynamics} The problem can be represented through a discrete event simulation. A state $x_t$ is defined by the set of waiting jobs and their features as above, and the current class attribution of the machines. Specifically, each machine is represented by the class of jobs it is currently set-up for, whether they are currently occupied by some job, and if so, the remaining processing time. The matrix of setup change times is also observable. A state is treated as a decision point if there are at least one free machine and one waiting job in that state.

% Actions are represented by tuples $(j, m)$, corresponding to processing job $j$ on machine $m$. When the action is executed, an \emph{event}, representing an update to the state, is registered for the time when the job terminates.
%\jo{It is my understanding the noops are not allowed anymore, right? Also, this would be consistent with the cvrp env. in which noops are disallowed} \fr{we don't allow the trained policy to do noops, since that gave bad training results. We do however allow MCTS to choose noops.}
% Alternatively, a \texttt{noop} action can be executed that does not start a job on any of the free machines. In both cases, the simulation is iteratively fast-forwarded to the next event until the next decision point is reached.
% While slightly abusing notation, we define the immediate reward, $r_t$, as $\Gamma(x_{t+1}) - \Gamma(x_t)$, replacing the completion time with the current time of state $x$ for uncompleted jobs. Thus, the total reward of an episode is just the TWCT objective value since 
% \begin{equation*}
%     \sum_{t=0}^{T-1} r_t = \sum_{t=0}^{T-1} \left( \Gamma(x_{t+1}) - \Gamma(x_t) \right)
%     = \Gamma(x_{T}) - \Gamma(x_0) = \Gamma(x_{T}) = \Gamma(\mathbf{c}).
% \end{equation*}
%Note that $\Gamma(x_0) = 0$ and that $\Gamma(x_{T})$ is just the TWCT objective value.


\paragraph{The advantage of learning the input distribution} Many of the known baseline approaches for online variants are based on simple modifications that disregard the underlying arrival distributions. One would expect that a method adept at learning the arrival distribution, either explicitly or implicitly (as is the case for Q values) would improve upon such naive, myopic approaches~\cite{garg08}. In fact, one can prove that for both CVRP and scheduling, the competitive ratio between an online and an offline algorithm in an online setting can be arbitrarily high. Appendix~\ref{app:inputdistribution} contains a detailed discussion.


==> setup.tex <==
\section{Setup}
TBD............

==> static_cvrp_table.tex <==
\begin{table}[t]
    \caption{Resutls for offline CVRP problem of different sizes.}
    \label{tab:totalParams}
    \tiny
    \centering
    \begin{tabular}{l*3c}
        \toprule
        Baseline & VRP 20 & VRP 50 & VRP 100  \\ 
        \midrule
        Uniformly Random        & -13.21 (107.51\%) & -30.58 (167.52\%)         & -58.84 (230.13\%) \\
        Distance Proportional   & -10.43 (63.65\%)  & -24.36 (113.39\%)         & -47.59 (167.38\%) \\
        Savings                 & -6.35 (-1.04\%)   & \textbf{-11.03 (-3.98\%)} & \textbf{-16.51 (-7.94\%)} \\
        Sweep                   & -8.89 (39.33\%)   & -17.23 (49.94\%)          & -28.24 (58.11\%) \\
        OR-Tools                & -6.42 (0.00\%)    & -11.50 (0.00\%)           & -17.96 (0.00\%) \\
        Neural-Rewriter         & -6.95 (8.48\%)    & -12.83 (11.83\%)          & -19.45 (8.57\%) \\
        Q-net                   & -6.84 (6.59\%)    & -12.33 (7.37\%)           & -19.27 (7.62\%) \\
        MCTS+random             & -7.65 (19.45\%)   & -20.72 (81.08\%)          & -46.34 (160.11\%) \\
        MCTS+distance           & -7.15 (12.01\%)   & -18.91 (65.04\%)          & -44.00 (147.44\%) \\
        \textbf{SOLO}           & \textbf{-6.21 (-3.18\%)} & -11.25 (-1.98\%) & -17.68 (-1.24\%) \\
        \bottomrule
    \end{tabular}
\end{table}


==> static_pms_table.tex <==
% \begin{table}[t]
%     \caption{Resutls for offline CVRP problem of different sizes.}
%     \label{tab:totalParams}
%     \tiny
%     \centring
%     \begin{tabular}{l*2c}
%         \toprule
%         {} & Liao 20 & Liao 80  \\ 
%         \midrule
%         WSPT                & -16570.16 (5.84\%)          & -182357.02 (4.15\%)         \\
%         CPLEX               & -15658.46 (0.00\%)          & -175084.88 (0.00\%)         \\
%         Neural-Rewriter     & -16540.28 (5.64\%)          & -182450.02 (4.20\%)         \\
%         MCTS+WSPT           & -15876.88 (1.42\%)          & -176439.74 (0.74\%)         \\
%         Q-net               & -15906.32 (1.57\%)          & -178444.74 (1.95\%)         \\
%         \textbf{SOLO}       & -15695.94 (0.25\%)          & -175524.34 (0.24\%)         \\
%         \textbf{SOLO+Prune} & -15683.46 (0.20\%)          & -175164.58 (0.05\%)         \\
%         optimal             & -15628.68 (-0.17\%)         & \multicolumn{1}{c}{-}       \\
%         \bottomrule
%     \end{tabular}
% \end{table}

%                 & \multicolumn{1}{c}{Liao 20} & \multicolumn{1}{c}{Liao 80} \\

% WSPT                & -16570.16 (5.84\%)          & -182357.02 (4.15\%)         \\
% CPLEX               & -15658.46 (0.00\%)          & -175084.88 (0.00\%)         \\
% Neural-Rewriter     & -16540.28 (5.64\%)          & -182450.02 (4.20\%)         \\
% MCTS+WSPT           & -15876.88 (1.42\%)          & -176439.74 (0.74\%)         \\
% Q-net               & -15906.32 (1.57\%)          & -178444.74 (1.95\%)         \\
% \textbf{SOLO}       & -15695.94 (0.25\%)          & -175524.34 (0.24\%)         \\
% \textbf{SOLO+Prune} & -15683.46 (0.20\%)          & -175164.58 (0.05\%)         \\
% optimal             & -15628.68 (-0.17\%)         & \multicolumn{1}{c}{-}       \\




\begin{table}[]
\caption{Scheduling results for all problem variants. Each cell includes the average cost on 50 seeds and the fractional improvement of each method compared to CPLEX (negative numbers are better than CPLEX).}
\label{tab:scheduling_results}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{@{}lllll@{}}
\toprule
                & \multicolumn{2}{c}{Online}                                       & \multicolumn{2}{c}{Offline}                               \\ \midrule
                & \multicolumn{1}{c}{10 machines} & \multicolumn{1}{c}{3 machines} & \multicolumn{1}{c}{Liao 20} & \multicolumn{1}{c}{Liao 80} \\
Q-net           & -26031.50 (6.55\%)              & -37386.90 (5.83\%)             & -15906.32 (1.57\%)          & -178444.74 (1.95\%)         \\
SOLO            & -24747.38 (1.03\%)              & -35434.46 (0.30\%)             & -15695.94 (0.25\%)          & -175524.34 (0.24\%)         \\
SOLO+Prune      & -24655.42 (0.89\%)              & -35280.20 (-0.09\%)            & -15683.46 (0.20\%)          & -175164.58 (0.05\%)         \\
MCTS+WSPT       & -24724.76 (1.12\%)              & -35489.56 (0.59\%)             & -15876.88 (1.42\%)          & -176439.74 (0.74\%)         \\
WSPT            & -29102.50 (19.18\%)             & -40601.34 (14.76\%)            & -16570.16 (5.84\%)          & -182357.02 (4.15\%)         \\
CPLEX           & -24481.90 (0.00\%)              & -35294.38 (0.00\%)             & -15658.46 (0.00\%)          & -175084.88 (0.00\%)         \\
neural rewriter & -27350.68 (12.30\%)             & -38575.78 (9.10\%)             & -16540.28 (5.64\%)          & -182450.02 (4.20\%)         \\
optimal         & \multicolumn{1}{c}{-}           & \multicolumn{1}{c}{-}          & -15628.68 (-0.17\%)         & \multicolumn{1}{c}{-}       \\ \bottomrule
\end{tabular}
}
\end{table}

==> static_table.tex <==
\begin{table}[t]
    \caption{Offline results}
    \begin{minipage}{.5\linewidth}
    \caption{CVRP}
    % \label{tab:totalParams}
    \tiny
    \centering
        \begin{tabular}{l*3c}
            \toprule
            {} & VRP 20 & VRP 50 & VRP 100  \\ 
            \midrule
            Uniformly Random        & -13.21 (107.51\%) & -30.58 (167.52\%)         & -58.84 (230.13\%) \\
            Distance Proportional   & -10.43 (63.65\%)  & -24.36 (113.39\%)         & -47.59 (167.38\%) \\
            Savings                 & -6.35 (-1.04\%)   & \textbf{-11.03 (-3.98\%)} & \textbf{-16.51 (-7.94\%)} \\
            Sweep                   & -8.89 (39.33\%)   & -17.23 (49.94\%)          & -28.24 (58.11\%) \\
            OR-Tools                & -6.42 (0.00\%)    & -11.50 (0.00\%)           & -17.96 (0.00\%) \\
            Neural-Rewriter         & -6.95 (8.48\%)    & -12.83 (11.83\%)          & -19.45 (8.57\%) \\
            Q-net                   & -6.84 (6.59\%)    & -12.33 (7.37\%)           & -19.27 (7.62\%) \\
            MCTS+random             & -7.65 (19.45\%)   & -20.72 (81.08\%)          & -46.34 (160.11\%) \\
            MCTS+distance           & -7.15 (12.01\%)   & -18.91 (65.04\%)          & -44.00 (147.44\%) \\
            \textbf{SOLO}           & \textbf{-6.21 (-3.18\%)} & -11.25 (-1.98\%) & -17.68 (-1.24\%) \\
            \bottomrule
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
    \caption{PMS}
    % \label{tab:totalParams}
    \tiny
    \centering
        \begin{tabular}{l*2c}
            \toprule
            {} & Liao 20 & Liao 80  \\ 
            \midrule
            WSPT                & -16570.16 (5.84\%)          & -182357.02 (4.15\%)         \\
            CPLEX               & -15658.46 (0.00\%)          & -175084.88 (0.00\%)         \\
            Neural-Rewriter     & -16540.28 (5.64\%)          & -182450.02 (4.20\%)         \\
            MCTS+WSPT           & -15876.88 (1.42\%)          & -176439.74 (0.74\%)         \\
            Q-net               & -15906.32 (1.57\%)          & -178444.74 (1.95\%)         \\
            \textbf{SOLO}       & -15695.94 (0.25\%)          & -175524.34 (0.24\%)         \\
            \textbf{SOLO+Prune} & -15683.46 (0.20\%)          & -175164.58 (0.05\%)         \\
            optimal             & -15628.68 (-0.17\%)         & - \\
            \bottomrule
        \end{tabular}
    \end{minipage}

\end{table}

==> training_time.tex <==
\begin{table}[t]
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{lll}%
        \textbf{Problem} & \textbf{GPUh} & \textbf{Resources} \\
        CVRP Offline size $20$  & $13.08$ & \multirow{2}{*}{\shortstack[l]{$18$-core Intel \\ Xeon Gold $6150$ @ $2.70$ GHz \\ Nvidia Tesla V$100$ ($16$ GB)}} \\ 
        CVRP Offline size $50$  & $14.68$ \\
        CVRP Offline size $100$ & $20.46$ \\[5pt]
        \hline \\
        CVRP Online size $20$   & $5.08$ & \multirow{2}{*}{\shortstack[l]{20-core Intel i9-10900X @ 3.70GHz \\ Nvidia GeForce RTX 2080 (11 GB)}} \\ 
        CVRP Online size $50$   & $17.05$ \\
        CVRP Online size $100$  & $7.38$ \\[5pt]
        \hline \\
        PMS Offline size $20$   & $14.3$ & \multirow{2}{*}{\shortstack[l]{$18$-core Intel\\ Xeon Gold $6150$ @ $2.70$ GHz \\ Nvidia Tesla V$100$ ($16$ GB)}}\\
        PMS Offline size $80$   & $21.83$ \\
        PMS Online $3$ machines & $6.9$ \\
        PMS Online $10$ machines& $10.65$ \\
    \end{tabular}%
    }
    \caption{Training time until the best model for the benchmark problems reported in GPU hours.}
    \label{tab:training_time}
\end{table}
% ($3.70$ GHz max. Turbo)
